FarSight: A Physics-Driven Whole-Body Biometric System at Large Distance and Altitude

Whole-body biometric recognition is an important area of research due to its vast applications in law enforcement, border security, and surveillance. This paper presents the end-to-end design, development and evaluation of FarSight, an innovative software system designed for whole-body (fusion of face, gait and body shape) biometric recognition. FarSight accepts videos from elevated platforms and drones as input and outputs a candidate list of identities from a gallery. The system is designed to address several challenges, including (i) low-quality imagery, (ii) large yaw and pitch angles, (iii) robust feature extraction to accommodate large intra-person variabilities and large inter-person similarities, and (iv) the large domain gap between training and test sets. FarSight combines the physics of imaging and deep learning models to enhance image restoration and biometric feature encoding. We test FarSight's effectiveness using the newly acquired IARPA Biometric Recognition and Identification at Altitude and Range (BRIAR) dataset. Notably, FarSight demonstrated a substantial performance increase on the BRIAR dataset, with gains of +11.82% Rank-20 identification and +11.3% TAR@1% FAR.

==> ref/figure_ref.tex <==
\begin{figure}[t!]
\begin{center}
\resizebox{1\linewidth}{!}{
\begin{tabular}{c c c c c}
{\includegraphics[height=3cm]
{fig/Feng/pairs/hs_genuine/BTS1.0_G00003_field_0000114712____BTS1_G00003_controlled_0000002844____1.0601.png}} & 
{\includegraphics[height=3cm]{fig/Feng/pairs/hs_genuine/BTS1.0_G00071_field_0000118399____BTS1_G00071_controlled_0000002938____1.143.png}} &
{\includegraphics[height=3cm]{fig/Feng/pairs/hs_genuine/BTS1.0_G00073_field_0000119810____BTS1_G00073_controlled_0000001413____1.1114.png}} &
{\includegraphics[height=3cm]{fig/Feng/pairs/hs_genuine/BTS1.0_G00293_field_0000136963____BTS1_G00293_controlled_0000004716____1.0602.png}} &
{\includegraphics[height=3cm]{fig/Feng/pairs/hs_genuine/BTS1.0_G00448_field_0000157658____BTS1_G00448_controlled_0000005519____1.1014.png}}  \\
\multicolumn{5}{c}{\LARGE (a) Successful Recognition of Genuine Pairs}\vspace{3mm}\\ 
{\includegraphics[height=3cm]{fig/Feng/pairs/ls_impostor/BTS1.0_G00083_field_0000121633____BTS2_G02678_controlled_0000041763____-0.60766.png}} & 
{\includegraphics[height=3cm]{fig/Feng/pairs/ls_impostor/BTS1.0_G00246_field_0000130545____BTS2_G02529_controlled_0000032686____-0.64466.png}} &
{\includegraphics[height=3cm]{fig/Feng/pairs/ls_impostor/BTS1.0_G00380_field_0000150022____BTS2_G02682_controlled_0000042160____-0.61029.png}} &
{\includegraphics[height=3cm]{fig/Feng/pairs/ls_impostor/BTS2.0_G02005_field_0000551568____BTS1_G00143_controlled_0000005168____-0.61122.png}} &
{\includegraphics[height=3cm]{fig/Feng/pairs/ls_impostor/BTS2.0_G02053_field_0000578230____BTS1_G00236_controlled_0000007772____-0.60312.png}}  \\
\multicolumn{5}{c}{\LARGE (b) Successful Recognition of Impostor Pairs}\vspace{3mm}\\
{\includegraphics[height=3cm]{fig/Feng/pairs/ls_genuine/BTS1.0_G00026_field_0000116303____BTS1_G00026_controlled_0000003233____-0.038741.png}} & 
{\includegraphics[height=3cm]{fig/Feng/pairs/ls_genuine/BTS1.0_G00162_field_0000123789____BTS1_G00162_controlled_0000012232____0.17941.png}} &
{\includegraphics[height=3cm]{fig/Feng/pairs/ls_genuine/BTS2.0_G02011_field_0000552533____BTS2_G02011_controlled_0000013408____0.20464.png}} &
{\includegraphics[height=3cm]{fig/Feng/pairs/ls_genuine/BTS2.0_G02052_field_0000575654____BTS2_G02052_controlled_0000007329____0.16695.png}} &
{\includegraphics[height=3cm]{fig/Feng/pairs/ls_genuine/BTS2.0_G02063_field_0000582889____BTS2_G02063_controlled_0000000524____0.17496.png}}  \\
\multicolumn{5}{c}{\LARGE (c) Failure Cases for Genuine Pairs}\vspace{3mm}\\
{\includegraphics[height=3cm]{fig/Feng/pairs/hs_impostor/BTS1.0_G00003_field_0000114924____BTS1_G00044_controlled_0000001130____1.0442.png}} & 
{\includegraphics[height=3cm]{fig/Feng/pairs/hs_impostor/BTS1.0_G00134_field_0000122985____BTS1_G00071_controlled_0000002938____1.0872.png}} &
{\includegraphics[height=3cm]{fig/Feng/pairs/hs_impostor/BTS1.0_G00286_field_0000136103____BTS1_G00124_controlled_0000004193____1.0882.png}} &
{\includegraphics[height=3cm]{fig/Feng/pairs/hs_impostor/BTS1.0_G00469_field_0000160417____BTS1_G00393_controlled_0000017635____1.0609.png}} &
{\includegraphics[height=3cm]{fig/Feng/pairs/hs_impostor/BTS1.0_G00550_field_0000169999____BTS1_G00304_controlled_0000008032____1.0825.png}}  \\
\multicolumn{5}{c}{\LARGE (d) Failure Cases for Impostor Pairs}\\
\end{tabular}
}
\end{center}
\vspace{-5mm}
\caption{\small Successful and failure examples of body matching.
} 
\label{fig:body_matching_paired_examples}
\vspace{-2mm}
\end{figure}


==> ref/ref.tex <==
\begin{table*}[t]
    \centering
\resizebox{0.98\linewidth}{!}{
    \begin{tabular}{|c||c|c|c||c|c|c|}
     \hline
      \multirow{2}{*}{Method} & \multicolumn{3}{c||}{Face Included} & \multicolumn{3}{c|}{Face Restricted} \\
      \cline{2-7}
      & \makecell{Verification\\TAR@$1$\% FAR $\uparrow$} & \makecell{Rank Retrieval\\Rank20 $\uparrow$} & \makecell{Open Search\\FNIR@$1$\% FPIR $\downarrow$} & \makecell{Verification\\TAR@$1$\% FAR $\uparrow$} & \makecell{Rank Retrieval\\Rank20 $\uparrow$} & \makecell{Open Search\\FNIR@$1$\% FPIR $\downarrow$} \\ 
      
     \hline\hline
 Baseline-ArcFace~\cite{}     & ?? & ?? & ?? & ?? & ?? & ?? \\       
 \textbf{FarSight-Face}    & ?? & ?? & ?? & ?? & ?? & ?? \\       
 Baseline-GaitBase~\cite{}    & ?? & ?? & ?? & ?? & ?? & ?? \\       
 \textbf{FarSight-Gait}    & ?? & ?? & ?? & ?? & ?? & ?? \\       
 Baseline-CAL~\cite{}         & ?? & ?? & ?? & ?? & ?? & ?? \\       
 \textbf{FarSight-Body}    & ?? & ?? & ?? & ?? & ?? & ?? \\    \hline
 \hline
  Baseline     & ?? & ?? & ?? & ?? & ?? & ?? \\
 \textbf{FarSight}     & ?? & ?? & ?? & ?? & ?? & ?? \\
 \hline
    \end{tabular}
    }
        \caption{Whole body biometric recognition results on the BRIAR dataset.}
	\label{tab:bts_results}
\end{table*}

\begin{table}
    \centering
    \begin{tabular}{|c|c|}\hline
        Module & Duration (seconds) \\
        \hline
        \emph{Detection \& Tracking} & $34.7$ \\ \hline
        \emph{Restoration}           & $5.3$ \\ \hline
        \emph{Face}                  & $2.2$ \\ \hline
        \emph{Gait}                  & $2.5$ \\ \hline
        \emph{Body}                  & $3.1$ \\ \hline
        \hline
    \end{tabular}
    \caption[4k Processing Time]{4k Processing Time}
    \label{tab:4k_processing_time}
\end{table}

\begin{table}
    \centering
    \begin{tabular}{|c|c|}\hline
        Module & Duration (seconds) \\
        \hline
        \emph{Detection \& Tracking}   & $24.9$ \\ \hline
        \emph{Restoration} & $5.9$ \\ \hline
        \emph{Face}        & $2.5$ \\ \hline
        \emph{Gait}        & $3.0$ \\ \hline
        \emph{Body}        & $3.5$ \\ \hline
    \end{tabular}
    \caption[Average Combined Processing Time]{Average Combined Processing Time}
    \label{tab:combined_average_processing_time}
\end{table}

\begin{table}
    \centering
    \begin{tabular}{|c||c|}\hline
        Media              & Pipeline total \\ \hline
        \emph{1080p Video} & $8.4$ fps\\ \hline
        \emph{4k Video}    & $6.3$ fps\\ \hline
        Average Combined   & $7.8$ fps \\ \hline
    \end{tabular}
    \caption[Average Pipeline FPS]{Average Pipeline fps.}
    \label{tab:speed_pipeline}
\end{table}

==> ref/sec_3_method_v1.tex <==

\begin{figure*}[t]
\begin{center}
%\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
\includegraphics[width=0.9\linewidth]{fig/Feng/fig2_overview.pdf}
\end{center}
   \caption{Illustration of FarSight system.}
\label{fig:overview}
\end{figure*}

\section{FarSight: System Architecture}\label{sec:}

\subsection{Overview of FarSight}
% {\color{red} [Chris, MSU]}
%%
As shown in Fig.~\ref{fig:overview}, the FarSight system operates through an intricate assembly of six modules, each tailored for a specific function: detection and tracking, image restoration, three biometric modalities, namely, face, gait, and body feature extraction, and multi-modality fusion module. These modules function within a containerized testing framework, utilizing GPU resources effectively through dynamically adjustable batch sizes.

%%
An API utility bridges the interaction between the framework and external systems, streaming video sequences identified from configuration files to the testing framework using Google RPC calls. The framework then extracts vital features from these sequences, which are stored in HDF5 databases for match performance evaluation.


%%
The workflow begins with video sequence processing through the detection and tracking modules. Bounding box-detected images are cropped and dispatched to the gait and body feature encoding module. Simultaneously, the cropped face frames undergo image restoration before their delivery to the face module. 
%
Both the body and gait modules produce a unique per-sequence feature vector from a single run of all sequences via average pooling operation, while the face pipeline employs CAFace~\cite{caface} to aggregate the features across various sequences.

%The body and gait modules yield a singular per-sequence feature vector from a single pass of all sequences, while the face pipeline adopts CAFace to aggratee the features across features.

%a two-stage process. This process first produces intermediate AdaFace feature vectors for each frame, which are then refined by CAFace to generate the final feature vector.

%%
Catering to the varying needs of enrollments, the system processes probe enrollments as single video segments per subject, generating definitive feature vectors. Conversely, gallery enrollments, composed of multiple video sequences and still images, undergo additional consolidation, merging into a singular, comprehensive subject-level feature vector post-processing.

%\noindent 
%The FarSight system is comprised of five modules that provide functions for detection and tracking, image restoration, and the three biometric modalities: body extraction, face extraction and gait extraction.  Each module is wrapped in a standard interface and deployed in containerized testing framework.

%The testing framework listens for calls to standard functions for gallery and probe enrollment into a database, database manipulation functions for merging and finalizing, and scoring functions to generate raw matching data that can subsequently be processed to generate performance results.

%Calls to the testing framework originate via an API utility that takes configuration files that identify gallery and probe source media and streams media to the testing framework over Google RPC calls in a frame-by-frame manner.  Still images (gallery only) and videos (both gallery and probe) are submitted to the test framework for feature extraction and the framework writes extracted features out to databases in the HDF5 format. These databases can then be utilized to determine matching performance.

%Each module is executed asynchronously in its own process space, allowing for different batch sizes for each module to make best use of available GPU resources.  Results are synchronized at the end of processing of each media piece.

%Media is first sent to the detection and tracking modules and fed to subsequent modules, following appropriate pre-processing, as detection and tracking results become available.  Frame-by-frame image data and corresponding detection bounds are first pre-processed into appropriately cropped and scaled batches before sending to the body and gait modules.  Image restoration is applied to face frames before sending to the face module.  Both restored and unrestored imagery is sent to the face module to allow it to make a best-result judgement on which form to use.

%Body and gait both process all images in each discrete media in a single pass resulting in a single per-media feature vector respectively.  In contrast, the face pipeline processes in two stages, first generating intermediate AdaFace feature vectors for each frame in the source media, and then passing those intermediate feature vectors to CAFace to generate a resulting feature vector.

%Probe enrollments consist of a single video segment per subject, and thus the resulting feature vectors above are final.  Gallery enrollments, however, consist of multiple video and still images and the media-level feature vectors must be finalized into a single subject-level feature vector once all gallery media has been processed.
%Fig.~\ref{fig:overview} 


\begin{figure}[t]
\begin{center}
\includegraphics[width=0.95\linewidth]{fig/Feng/fig3_briar_examples.pdf}
\end{center}
   \caption{The examples in the BRIAR dataset~\cite{cornett2023expanding} illustrate a subject under various conditions, including different distances, clothing, and varying quality due to the turbulence effect. The columns represent different scenarios: controlled conditions, close range, 100m-set1, 100m-set2, 200m, 400m, 500m, and UAV respectively. The subjects in the figure (ID: G02030, G02062, G02217 and G02229) consented to publication.}
\label{fig:briar_examples}
\end{figure}

\subsection{Challenges in Long-Distance and High-Altitude Recognition }
%{\color{red} [Feng, MSU]}

Our FarSight system faces an array of unique challenges.
%
Firstly, long-range capture and atmospheric turbulence often result in low-quality biometric samples that are difficult to process. Secondly, elevated platforms introduce large yaw and pitch angles, further complicating the data analysis. Additionally, the low visual quality hampers the extraction of identity information, making accurate recognition more difficult. The training data also presents a limitation, as its domain is restricted due to diverse environmental changes. Lastly, the low generalizability and explainability of deep learning models pose a significant challenge to the achievement of reliable and transparent results. 
%
In Fig.~\ref{fig:briar_examples}, we provide examples from close-range, mid-range (100m-500m), and UAV scenarios for a more visual understanding of these challenges. 

\subsection{Physics Modeling of Turbulence}

\noindent Atmospheric turbulence is an unavoidable degradation when imaging at range. It is often computationally modeled by splitting the continuous propagation paths into segments via phase screens as illustrated in Fig.~\ref{fig: turbulence simulation}. 
While accurate, the spatially varying nature of the propagation
%For \emph{every} point on the object plane, we need to perform a series of Fourier transforms and phase multiplications to compute the point spread function on the image plane \cite{Hardie_2017_a, Hardie_2022_a, Schmidt_2010_a}. 
makes this a computationally expensive process \cite{Hardie_2017_a, Hardie_2022_a, Schmidt_2010_a}.



\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{./fig/turbulence/turb_simulation}
\caption{Comparing split-step and Zernike-based simulations \cite{Chimitt_2020_a, Mao_2021_a, chimitt_2022_a}.}
\label{fig: turbulence simulation}
\end{figure}


More recent works have explored the possibility of \emph{propagation-free} models where the turbulence effects are implemented as random sampling at the \emph{aperture} \cite{Chimitt_2020_a, Mao_2021_a, chimitt_2022_a}. As shown in Fig.~\ref{fig: turbulence simulation}, every pixel on the aperture is associated with a random phase function which has a linear representation using the Zernike polynomials \cite{Noll_1976_a}. By constructing the covariance matrix of the random process, we can draw samples of the Zernike coefficients to enforce spatial and modal correlations. Propagation-free simulation has enabled $1000 \times $ speed up compared to the split-step propagation methods while maintaining the accuracy. Therefore, we adopt this simulation appraoch in our system.
%This will lead to two principal components of the turbulent effects: (1) tilt (i.e., geometric displacement of pixels) and (2) spatially varying blur \cite{Chan_2022_a},
% \begin{equation}
%     I(\mathbf{x}) = [\mathcal{B} \circ \mathcal{T}] (J(\mathbf{x})),
%     \label{eq: turb_img_form}
% \end{equation}
% where $\mathcal{T}$ is the tilt operator and $\mathcal{B}$ represents the blur operation, with $J(\mathbf{x})$ and $I(\mathbf{x})$ as the input and output images, indexed by position $\mathbf{x}$, respectively. 




For the generation of training data, realistic optical and turbulence parameters significantly influence the appearance of the generate defects. Therefore, our datasets are synthesized according to the metadata of various long-range optical systems. Our training dataset also consists of both dynamic and static scenes \cite{Safdarnejad_2015_a, Jin_2021_a, zhou2017places}. 


 %Solving the inverse problem of \eqref{eq: turb_img_form} is highly non-trivial and deviates from many classical deblurring problems \textcolor{red}{[a few citations]}, where blur is assumed to be uniform or the shifting to be global. 


% For learning-based restoration, imaging through turbulence poses a significant problem: ground truth is almost \emph{never} available -- if the image is observed through turbulence at one instance, we cannot ``turn it off'' in the next. Therefore, reliance on simulation for restoration is essential. Although existing methodologies exist \textcolor{red}{[split-step works]}, generating a sufficient amount of data is likely infeasible as noted by Chimitt et al. .
% %the generation a 4k dataset consisting of 1000 sequences with 100 frames each will take 156 years to process using split-step based methods.



%The series of works describing Zernike-based simulation  succeed in maintaining accuracy while increasing the speed by a factor of $\times\!1000$. Although the capability exists, proper selection of parameters and application to images in training is non-trivial. Improper application will overemphasize certain aspects such as pixel shifting or blur size, therefore, to accurately represent imaging through turbulence, we must choose the parameters carefully. Because we are specifically interested in biometric recognition, we can tailor our parameter choices for simulation to reasonably match our expectation for where our restoration may be applied. Exact parameter choices can be found in the supplementary document. The types of scenes we focus are fairly general, simulating on a few video datasets \cite{Safdarnejad_2015_a, Jin_2021_a, zhou2017places}.






\subsection{Detection and Tracking {\color{green} [UO team]}}
%%%% Will redo equations to avoid overflowing
%%%% Figures will be added soon.
Herein, we describe our detection module, which is based on the joint body and face detection method proposed by Wan et al.~\cite{wan2021bodyface}.
This detection framework is designed to associate detected face bounding boxes with body bounding boxes, making it more convenient for handing off bounding boxes to biometric models.

The framework consists of a two-stage R-CNN-based~\cite{ren2015faster} detector with a slightly modified ResNet50 backbone.
It performs a binary detection task (face or body) on proposed regions, and later associates face and body bounding boxes.
Association can be challenging due to the fact that face and body detection outputs lack the necessary level of correlation to assist pairwise matching.
The joint detection framework we use~\cite{wan2021bodyface} builds on learning associative embeddings~\cite{newell2017associative}, and introduces a second learnable embedding branch, which is optimized by ground truth identifiers.
In addition to learning embeddings, the framework also learns to predict a ``head hook'' coordinate from the center of face bounding boxes. 
Body and face bounding boxes are finally associated through a combination of associative embedding similarities, confidence scores, and head hook distances.

\subsubsection{Associative embedding}
Let $\mathcal{G}$ be the set of ground truth annotations:
\begin{equation*}
    \mathcal{G} = \{(g_1^{(b)},g_1^{(f)}), (g_2^{(b)},g_2^{(bf}), \dots, (g_S^{(b)},g_S^{(f)})\} \ ,
\end{equation*}
where $(g_k^{(b)},g_k^{(f)})$ represents the pair of body and face annotations of the $k$-th subject, and $S$ is the number of subjects. 
We separate all detected boxes into two disjoint sets: body boxes ($\mathbf{B}$), and face boxes ($\mathbf{F}$). 
The algorithm matches body and face proposals with subjects based on an overlap threshold.
We denote $\mathbf{B}_k$ and $\mathbf{F}_k$ be the set of body and face proposals for the ground truth body and face boxes of the $k$-th subject respectively:
\begin{equation*}
    \mathbf{B}_k = \{ b_i \in \mathbf{B} \ | \ IoU(b_i, g_k^{(b)}) > \eta \} \ ,
\end{equation*}
\begin{equation*}
    \mathbf{F}_k = \{ b_i \in \mathbf{F} \ | \ IoU(b_i, g_k^{(f)}) > \eta \} \ ,
\end{equation*}
where $\eta$ is the overlap threshold. 

As previously pointed out, the framework is designed to learn a second set of embeddings for every region of interest in order to associate face and body predictions.
For every box proposal $b$, it learns $l_2$-normalized embeddings, $f(b)$, which are used to associate pairs of face and body boxes that could be of the same subject. 

These associative embeddings are learned from two loss functions: a \textbf{Pulling Loss} and a \textbf{Pushing Loss}. 
As the names suggest, the former attempts to map embeddings of the same subject closer, whereas the latter pushes those embeddings of different subjects away. 

\Paragraph{Pulling loss}
Pulling loss is defined for pairs of bounding boxes, which can be either body-to-body, face-to-face, and face-to-body pairs.
Pulling loss for body-to-body pairs is calculated as follows:
\begin{align}
    &L_{bb}^{pull} = \nonumber \\
    &\frac{1}{S} \sum_{k=1}^{S}{ \frac{1}{{| \mathbf{B}_k |}^2} \sum_{x \in \mathbf{B}_k}\sum_{\substack{y \in \mathbf{B}_k\\y \neq x}} \exp{(dist(x, y))} \parallel f(x) - f(y) \parallel^2 } \ ,
\end{align}
where the $dist$ is the distance function between the center points of proposals. 
Pulling loss for face-to-face pairs is calculated similarly:
\begin{align}
    &L_{ff}^{pull} = \nonumber \\
    &\frac{1}{S} \sum_{k=1}^{S}{ \frac{1}{{| \mathbf{F}_k |}^2} \sum_{x \in \mathbf{F}_k}\sum_{\substack{y \in \mathbf{F}_k\\y \neq x}} \exp{(dist(x, y))} \parallel f(x) - f(y) \parallel^2 } \ .
\end{align}

Body-to-face pairs are calculated similarly, with the exception of not including distance-aware weighting. 
This is simply because the face bounding box of one subject can actually be closer to another subject's body bounding box. 
Therefore the body-to-face pull loss is calculated as follows:
\begin{equation}
    L_{bf}^{pull} = \frac{1}{S} \sum_{k=1}^{S}{ \frac{1}{| \mathbf{B}_k || \mathbf{F}_k |} \sum_{x \in \mathbf{B}_k}{\sum_{y \in \mathbf{F}_k}{ \parallel f(x) - f(y) \parallel^2 } } } \ .
\end{equation}
The total pulling loss is then calculated as a weighted sum of the body-to-face loss, and the sum of the face-to-face and body-to-body losses:
\begin{equation}
    L^{pull} = \mu L_{bf}^{pull} + \beta(L_{bb}^{pull} + L_{ff}^{pull}) \ .
\end{equation}

\Paragraph{Pushing loss}
This loss focuses on pushing bounding boxes assigned to different subjects away, and like pulling loss is divided into three losses between pairs of body boxes, pairs of face boxes, and body-face pairs.

\begin{align}
    &L_{bb}^{push} = \nonumber \\
    &\frac{1}{S^2} \sum_{k=1}^{S}{ \sum_{\substack{l=1\\l \neq k}}^{S}{ \frac{1}{|\mathbf{B}_k||\mathbf{B}_l|} \sum_{x \in \mathbf{B}_k}\sum_{y \in \mathbf{B}_l} \max{(0, \delta - \parallel f(x) - f(y) \parallel^2)} }} \ ,
\end{align}
\begin{align}
    &L_{ff}^{push} = \nonumber \\
    &\frac{1}{S^2} \sum_{k=1}^{S}{ \sum_{\substack{l=1\\l \neq k}}^{S}{ \frac{1}{|\mathbf{F}_k||\mathbf{F}_l|} \sum_{x \in \mathbf{F}_k}\sum_{y \in \mathbf{F}_l} \max{(0, \delta - \parallel f(x) - f(y) \parallel^2)} }} \ ,
\end{align}
\begin{align}
    &L_{bf}^{push} = \nonumber \\
    &\frac{1}{S^2} \sum_{k=1}^{S}{ \sum_{\substack{l=1\\l \neq k}}^{S}{ \frac{1}{|\mathbf{B}_k||\mathbf{F}_l|} \sum_{x \in \mathbf{B}_k}\sum_{y \in \mathbf{F}_l} \max{(0, \delta - \parallel f(x) - f(y) \parallel^2)} }} \ ,
\end{align}
where $\delta$ is the margin. 
Similar to the pulling loss, the three losses above are aggregated through a weighted sum:
\begin{equation}
    L^{push} = \mu L_{bf}^{push} + \beta (L_{bb}^{push} + L_{ff}^{push})
\end{equation}

\Paragraph{Final associative embedding loss}
The final loss used to optimize associative embeddings is a weighted sum of the pulling and pushing losses:
\begin{equation}
    Loss_{em} = \sigma L^{pull}  + \tau L^{push} \ .
\end{equation}

\subsubsection{Head hook prediction}
In addition to associative embeddings, the framework also predicts ``head hook'' coordinates for every subject, which further improves body and face association. 
Regardless of whether a ground truth subject has a face annotation or not, the joint detector is designed to predict a head hook, and optimizes it according to the ground truth head and body annotations. 
We denote the center of the ground truth head box of the $k^{th}$ subject as $h_k^*$, and the predicted head hook for the proposal associated with that subject as $h_k$.
The head hook loss is the weighted sum of the Smooth L1 loss~\cite{girshick2015fast} and a scale-invariant angular loss. The former is calculated as follows:
\begin{equation}
    Loss_{l1} = \frac{1}{\mathbf{|S|}}\sum_{k=1}^\mathbf{|S|}\sum_{h \in \mathbf{H_k}} \sum_{i \in \{ x, y \}} smooth_{L_1}(h_i, {h_k^*}_i) \ ,
\end{equation}
where $\mathbf{H_k}$ denotes the set of all head hooks whose bounding boxes are associated with subject $k$ (based on IoU), and: 
\begin{equation*}
    smooth_{L_1}(x, y) = 
    \begin{cases}
      0.5(x - y)^2 & |x-y|< 1 \\
      |x-y| - 0.5 & otherwise \ ,
    \end{cases}
\end{equation*}

The angular loss is computed as follows:
\begin{equation}
    Loss_{al} = \frac{1}{\mathbf{|S|}}\sum_{k=1}^\mathbf{|S|}\sum_{h \in \mathbf{H_k}}\frac{\parallel v_k(h) \times v_k(h_k^*) \parallel}{\parallel v_k(h) \parallel \times \parallel v_k(h_k^*) \parallel} \ ,
\end{equation}
where $v_k(h)$ is a vector originating from the center of the ground truth body box $g_k^{(b)}$, to predicted head hook coordinates $h$, and similarly $v_k(h_k^*)$ is a vector from the same origin to the ground truth head center $h_k^*$. 

\begin{equation}
    Loss_{hook} = \alpha Loss_{l1} + \gamma Loss_{al} \ .
\end{equation}

\subsubsection{Association}
Head hooks and embeddings from the earlier two stages help construct a similarity metric, through which the model associates body and face bounding boxes.
The similarity metric is comprised of three different metrics: embedding distance, head hook distance, and confidence scores.

\Paragraph{Embedding distance}
This is simply the RBF (radial basis function) kernel between detection embeddings classified as body and face.
We denote it with $\mathbf{M_e} \in \mathbb{R}^{|B| \times |F|}$.

\Paragraph{Head hook distance}
Similar to embedding distance, head hook distances are also an RBF kernel. 
The difference is that head hooks are simply 2-dimensional coordinates, whereas the embedding vectors were 32-dimensional. 
We denote pair-wise head hook distances with $\mathbf{M_h} \in \mathbb{R}^{|B| \times |F|}$.

\Paragraph{Confidence scores}
Confidence scores are an important metric in this particular case. 
As a result, they are directly included in the association loss to decrease the likelihood of associating a low-confidence bounding box with high-confidence one.
The pair-wise confidence score matrix is denoted with $\mathbf{P} \in \mathbb{R}^{|B| \times |F|}$, where:

\begin{equation}
    \mathbf{P}_{ij} = \frac{(C^b_i +C^f_j)^2}{2} \quad i=1,2,...,|B| \ , \  j=1,2,...,|F| \ ,
\end{equation}
where $C^b_i$ and $C^f_j$ are the $i$-th body and $j$-th face prediction confidence scores respectively. 

\Paragraph{Final association metric}
\begin{equation}
    \mathcal{S} = \mathbf{P} \otimes \mathbf{M}_h + (\mathbf{J_{|B|,|F|}} - \mathbf{P}) \otimes \mathbf{M}_e \ ,
\end{equation}
where $\otimes$ denotes Hadamard product, and $\mathbf{J_{|B|,|F|}}$ denotes the $|B|\times|F|$ ones matrix. 
After computing $\mathcal{S}$, every face prediction is associated with the body with which it has the maximum similarity. 
If the maximum similarity score is below the threshold ($0.98$ in our use case), it is concluded that the subject's face is not visible.
















\subsection{Image Restoration} 

\noindent At a high level, the image restoration task aims to invert the forward image formation process which has been mathematically described as \cite{Chan_2022_a},
\begin{equation}
    I(\mathbf{x}) = [\mathcal{B} \circ \mathcal{T}] (J(\mathbf{x})),
    \label{eq: turb_img_form}
\end{equation}
where $\mathcal{T}$ is the tilt operator and $\mathcal{B}$ represents the blur operation, with $J(\mathbf{x})$ and $I(\mathbf{x})$ as the input and output images, indexed by position $\mathbf{x}$, respectively. 
In this work, we have considered a single-frame image restoration method as well as a multi-frame method, both aiming to invert $\mathcal{T}$ and $\mathcal{B}$. %Although the forward model \eqref{eq: turb_img_form} is tilt-then-blur, for reconstruction it is easier to approximate this as blur-then-tilt.






%\noindent Image restoration seeks to invert the forward process of \eqref{eq: turb_img_form}. The first insight, following the lines of Chan \cite{Chan_2022_a}, is to note that for \emph{natural} images,
% \begin{equation}
%     [\mathcal{B} \circ \mathcal{T}] ( J (\mathbf{x})) \approx [\mathcal{T} \circ \mathcal{B}] ( J (\mathbf{x})). 
% \end{equation}
% Though \cite{Chan_2022_a} provides the reasoning as to why, we note that the approximation (i.e. blur-then-tilt) is easier to invert. The reason for this is two-fold: (1) the pixel-shifting operator $\mathcal{T}$ occupies roughly $90\%$ of the atmospheric distortions \textcolor{red}{[Noll]}, therefore, it is reasonable to expect that finding the inverse will simplify the deblurring problem (2) the $\mathcal{T}$ operator corresponds to \emph{geometric} distortions, thus, a network trained to learn typical image structures, and invert them, can be expected to perform well in the presence of a small to moderate amount of blur. Therefore, our network can be divided conceptually into two components, an inverse tilt operator $\mathcal{T}^{-1}$ and an inverse blur operator $\mathcal{B}^{-1}$.






% Therefore, the critical questions for a restoration method are: (1) what kind of limitations in processing speed and computational complexity may be imposed on restoration for a system which is operating near real-time (2) should restoration be done in a single-frame or multi-frame manner (3) how should we design a restoration method to \emph{boost} downstream task performance?






\subsubsection{Restoration for Biometrics}
Recent restoration methods which utilize Generative Adversarial Networks (GANs) \cite{Goodfellow_2020_a} or diffusion \cite{Dhariwal_2021_a} inject information into the restoration process in a generative fashion. Although more details are visible in reconstruction, we do not wish to \emph{change} the identify of a person by over-hallucinating information into the image. The design philosophy of our reconstruction methods aim towards restoring the image while keeping the identity unchanged. Combined with real-time application, our methods should be fairly lightweight to allow for shorter inference time.





Because of our application specifically in biometrics, two possible routes in image restoration present themselves: single-frame and multi-frame restoration. Single-frame restoration is useful due to a lesser throughput, though it must rely on stronger priors. That being said, the strength of the prior must be low enough as to not change the identity of the subject. Multi-frame restoration, by contrast, can use a weaker prior by virtue of incorporation of temporal information which comes at the cost of a larger throughput. %\textcolor{red}{These should be updated to reflect performance of system (I think TurbNet is slower than RTM)}





% If we are interested in biometrics, it is reasonable to expect that temporal information will be of significance to a restoration pipeline. Neighboring frames may have information relevant to this current frame, such as a person's head facing the imaging device or the turbulence (by virtue of its inherent randomness) may by minimal at a particular instance in time. Multi-frame methods are advantageous over single-frame methods in this respect.










% In addition to these considerations, recent restoration methods such as Generative Adversarial Networks (GANs) or \textcolor{red}{[some other method]} inject information into the restoration process in a generative fashion. Though this may indeed produce more details that were not present in the original observation, we do not wish to \emph{change} the identify of a person by \emph{over}-hallucinating information into the image (not to mention implicit biases that may be present in the chosen generative method). Our restoration's lightweight philosophy is in line with these considerations: we do not wish to \emph{over} restore by hallucination at the cost of reduced performance in downstream tasks.




% With these requirements in mind, we aim to have a lightweight, multi-frame restoration method which utilizes minimal generative concepts. For this task, recurrent neural networks (RNNs) are positioned to aid in the incorporation of temporal information with minimal overhead. \textcolor{red}{A couple more sentences here. Not sure how much we want to overlap with RTM paper?}




\subsubsection{Network Architecture}
For the multi-frame approach, we consider a convolutional recurrent network to restore the images, called the Recurrent Turbulence Mitigation network (RTM). The system layout of the method is shown in Fig~\ref{fig: rtm}. The RTM is bi-directional, multi-scale, and has a novel embedding fusion layer Multi-head Temporal Channel self-attention (MTCSA), to enhance the temporal fusion. This is the first recurrent-based network for multi-frame turbulence mitigation problems, and it is highly efficient because of the parameter reuse among different frames and implicit temporal fusion. 
%Our network is able to process 30 frames per second on $640\times 480$ image sequences on a single Nvidia 3080Ti.

\begin{figure}[h]
    \centering
    \includegraphics[width = 0.9\linewidth]{fig/turbulence/RTM_simple.jpg}
    \caption{Multi-frame image restoration by the recurrent network for turbulence mitigation (RTM).}
    \label{fig: rtm}
\vspace{-3ex}
\end{figure}

%\textcolor{blue}{Ajay - I talked with Prof. Liu, RTM should be enough for this paper as it was delivered it in the system, still if required, more details can be added.}
For the single-frame method, we adopt the approach proposed by Mao et al. \cite{Mao_2022_a}, known as the turbulence mitigation network (TurbNet), with the system diagram shown in Fig~\ref{fig: TurbNet}. TurbNet introduces the concept of estimating turbulence distortion while performing image restoration. The idea is that after the restoration has predicted the estimate, the estimate is re-distorted by the distortion map so that we can compare how well the prediction of the image and the distortion map has been.

\begin{figure}[h]
    \centering
    \includegraphics[width = \linewidth]{fig/turbulence/main_arch_eccv}
    \caption{single-frame image restoration by TurbNet.}
    \label{fig: TurbNet}
\vspace{-3ex}
\end{figure}





% The overall architecture of our RNN reconstruction module is shaped as U-net \cite{ronneberger2015u}. The decoder uses residual channel attention blocks (CAB) \cite{woo2018cbam, zhang2018image} and transposed convolution as the upsampling layers. Features extracted at each level of the encoders are passed to the associated level of the decoder by skip connections.



% Consecutive frames of turbulent sequences have similar degradations. These correlations have to potential to span multiple frames as described by the Greenwood frequency \cite{roggeman}. Mitigating biases in reconstruction due to this temporal correlation may require long video sequences as inputs which window-based models such as \cite{Zhang_2022_a, Jin_2021_a} are not well suited for due to memory limitations.





% Our architecture of an RNN is well-suited to incorporate these temporal dynamics. The recurrence is applied in both forward and backward directions using two identical and independent encoders. We build the encoders with residual dense blocks (RDB) \cite{zhang2018residual}. We further utilize 5-frame joint processing through a modified temporal channel self-attention. Self-attentions (SA) are spatially variant operations, which match the nature of turbulence, but they are known for their inefficiency in terms of memory. Therefore, our self attention modules are modified using channel-wise embeddings which fuse and compress the representation. Precise details can be found in the supplementary document, however, we note that the proposed MTCSA uses fewer parameters than the ``transposed attention'' in \cite{Zamir_2021_Restormer}.



















% \subsubsection{Training Procedure}



% Further complicating the task of biometric-recognition oriented restoration is the fact that subjects are often \emph{dynamic}. Therefore, a network must recognize which motion is due to turbulence (i.e., random pixel shifting) and which motion is due to true motion by the subject. To this end, in training we utilize multi-scale tilt distortions and tilt-free simulation to train our $\mathcal{T}^{-1}$ operator to recognize object motion vs. subject motion. This is specifically facilitated by our synthesis process, training on a loss between fully degraded images and tilt-free images (i.e., only $\mathcal{B}$ has been applied). Our $\mathcal{B}^{-1}$ component of our restoration network is trained on residuals of the previous network and the ground truth. We provide a conceptual illustration of the training procedure in 











\subsection{Multi-Modal Biometric Feature Encoding} %{\color{red} [Ryan and Feng, MSU]}}

We describe here our methods for obtaining identifying biometric features from our face, gait and body matching modules, as well as the multi-modal fusion technique applied to generate fused scores for evaluation on the various metrics described in Sec. \ref{evaluation-metrics}.

\subsubsection{Face }
\label{face-feature-encoding}
%{\color{green} [Minchul, MSU]}

Herein, we describe our face recognition pipeline that incorporates the methods of AdaFace~\cite{kim2022adaface}, CAFace~\cite{caface}, and CFSM~\cite{liu2022cfsm}, creating a comprehensive approach to overcome the challenges of recognizing faces across varied image qualities with both image and video media.

Our pipeline initiates with AdaFace~\cite{kim2022adaface}, an adaptive loss function technique designed for handling low-quality face datasets. The framework uses image quality to adaptively modulate the emphasis on misclassified samples, a feature particularly effective for managing the wide range of image qualities.

Further enhancement of our pipeline involves the implementation of CAFace~\cite{caface}, a two-stage feature fusion paradigm that is indispensable for incorporating features across multiple frames. By assigning inputs to a limited number of global cluster centers and later fusing the clustered features, CAFace provides the ability to combine multiple frames while maintaining order invariance.

Lastly, our pipeline incorporates the Controllable Face Synthesis Model (CFSM)~\cite{liu2022cfsm}. Given the persistent challenge of domain gaps between semi-constrained training datasets and unconstrained testing scenarios, CFSM provides a solution by mimicking the target datasets' distribution in a style latent space. This face synthesis model allows for precise control over the diversity and degree of synthesis, and the pre-trained synthesis model is designed to be guided by the FR model, generating images that are more beneficial for FR model training. Crucially, this approach allows us to generate synthetic face images similar in style to the target evaluation datasets, bridging the gap between high-quality training data and lower-quality surveillance images.

The amalgamation of AdaFace, CAFace, and CFSM within our pipeline forms a comprehensive solution to the challenges of face recognition across a diverse range of image qualities. Through effective frame-level feature extraction, integration of these features, and controllable synthetic image generation, our approach achieves substantial improvements in face recognition tasks across both high and low-quality image datasets.

\subsubsection{Gait }
%{\color{red} [Yiyang, MSU]}

Gait recognition is a biometric technique that focuses on analyzing an individual's walking patterns and movements to identify and differentiate them from others. 
% Unlike other biometric modalities like facial recognition, gait patterns can be captured from a distance and/or altitude.
It is particularly advantageous for long-distance and high-altitude surveillance applications, such as surveillance cameras mounted on buildings and unmanned aerial vehicles (UAVs), due to its ability to capture and analyze gait patterns from a distance. 
Unlike other biometric modalities like facial recognition, gait recognition can work effectively even when the subject's face is obscured, making it valuable in long-range and aerial scenarios. 
Additionally, gait recognition takes advantage of the dynamic nature of walking, capturing the unique rhythm, pace, and motion characteristics exhibited by individuals while other biometric modalities such as face recognition and body matching primarily rely on static features.
Focusing on the inherent temporal cues of gait enhances the accuracy and reliability of biometric identification in scenarios where other modalities may fall short.

Through our observations, we have identified a limitation in the current state-of-the-art gait recognition models, specifically their predominant focus on extracting local gait features while neglecting the essential global correlations. These global correlations refer to the interdependencies between different body parts across various frames of a gait sequence. In order to address this limitation and enhance the discriminability of gait recognition, we propose an innovative framework named GlobalGait. This framework aims to enrich the local gait features by incorporating and leveraging the crucial global correlations, thereby improving the overall effectiveness and accuracy of gait recognition.

In particular, given an input sequence \(\left(\mathbf{I}_1, \mathbf{I}_2, \dots, \mathbf{I}_{N}\right)\), we first use a CNN backbone to extract local spatiotemporal features \(\mathbf{F}_{\mathit{backbone}}\), which is then divided into \(\mathbf{F}_{\mathit{source}}\) and \(\mathbf{F}_{\mathit{target}}\). 
We project the feature maps to tokens \(\mathbf{T}\) for each joint by sampling around each 2D joint. 
And then, we use a stack of multi-head self-attention layers to model the spatial and temporal correlations in the sequences. 

To provide additional supervision signals for mining global correlations, we instruct our model to reconstruct the target frame pixels based on source sequences and select the correct target sequence among a batch of candidates. 
The goal is to exploit the spatial and temporal correlations in gait recognition and have these supervision signals provide feedback so that the model can learn more discriminative gait features.


\subsubsection{Body}
% {\color{red} [Feng, MSU]}
%%
The body feature encoding is an essential element of identity representation, widely used in person re-identification (Re-ID), search and tracking. In this subtask, we will leverage the Re-ID search to effectively encode the static body features.
%
Person Re-ID aims to re-identify a query person from a large image collection, taken by multiple cameras at different times~\cite{ye2021deep,ahmed2015improved,zheng2015scalable,li2018harmonious}. 
%
It is challenging due to the geometric misalignment and appearance ambiguity caused by the diversity of human poses and their clothing.
Thus, it is crucial to develop effective solutions to extract static body features that are robust to body pose and cloth-changing variations. 


%%
To address these challenges, we posit that the most reliable cue for body matching is the $3$D naked (unclothed) body shape, if it can be accurately and discriminately estimated from a $2$D body image.
%
The challenge of reconstructing a $3$D naked body is significant due to confounding factors and the lack of supervision, such as paired images and $3$D naked body scans. However, taking inspiration from recent advancements in $3$D feature learning for face recognition~\cite{peng2017reconstruction,liu2018disentangling}, we propose a novel pipeline to disentangle identity (naked body) from non-identity components (pose, clothing shape and texture) of $3$D clothed humans. 


%%%%%%% ----------- Figure ------------  %%%%%%%%%%
\begin{figure}[t]
  \centering
  \includegraphics[width=1\linewidth]{fig/Feng/bm_flowchart.pdf}
   \caption{\small Overview of the proposed body feature encoding framework. In the body matching process, the identity shape features $\mathbf{z}_{id}$ is utilized for matching.}
   \label{fig:bm_flowchart}
   %\vspace{-2mm}
\end{figure}
%%%%%%% ----------- Figure ------------  %%%%%%%%%%

%%
In particular, as illustrated in Fig.~\ref{fig:bm_flowchart}, the proposed method relies on a new joint two-layer neural implicit function that represents $3$D humans, where identity, clothing shape, and texture components are represented in disentangled latent representations.
%
Formally, given a training set of $T$ images $\{\mathbf{I}_i\}_{i=1}^{T}$ and the corresponding identity labels $\{l_i\}_{i=1}^{T}$,
the image encoder $\mathcal{E}(\mathbf{I}):\mathbf{I}\xrightarrow{} \mathbf{z}_{id}, \mathbf{z}_{cloth}, \mathbf{z}_{tex}$ predicts the identity shape code of naked body $\mathbf{z}_{id}\in\mathbb{R}^{L_{id}}$, clothed shape code $\mathbf{z}_{cloth}\in\mathbb{R}^{L_{cloth}}$ and texture code $\mathbf{z}_{tex}\in\mathbb{R}^{L_{tex}}$. A joint two-layer implicit model decodes the latent codes to identity shape, clothing shape, and texture components, respectively. 
%
Additionally, PoseNet $\mathcal{P}$ predicts the camera projection $\mathbf{\Omega}$ and SMPL body pose $\mathbf{\theta}$: $(\mathbf{\Omega}, \mathbf{\theta}) = \mathcal{P}(\mathbf{I})$.
%
Mathematically, the learning objective is defined as:
\begin{equation}
\label{eqn:objective}
\argmin_{\mathcal{E},\mathcal{F},\mathcal{C},\mathcal{T}} \sum_{i=1}^T \left(\left|\hat{\mathbf{I}}_i -  \mathbf{I}_i\right|_1 
+ \mathcal{L}_{cla}(\mathbf{z}_{id},l_i)\right),
\end{equation}
where $\mathcal{L}_{cla}$ is the classification loss. $\hat{\mathbf{I}}$ is the rendered image.
%
This  objective enables us to jointly learn accurate $3$D clothed shape and discriminative shape for the naked body.

%%
We employ a combination of CAPE~\cite{ma2020learning} and THuman2.0~\cite{zheng2019deephuman} datasets to instruct our joint two-layer implicit model. Each scan is processed to yield SMPL naked shape code and joint locations. Each training sample is assigned its own identity shape code, clothing shape code, and texture code through autodecoding.
%
For inference, the encoder $\mathcal{E}$ processes body images and extracts the identity shape features $\mathbf{z}_{id}$. The Cosine similarity of $\mathbf{z}_{id}$ is then used to determine if the two images belong to the same person. It is worth noting that, as the $3$D reconstruction module is not involved in this inference, it is highly efficient.

\subsubsection{Multi-Modality Fusion}
% {\color{red} [Ryan]}

To generate a probe-gallery score from multiple biometric modalities, first per modality scores are computed for all probe-gallery pairs. Each Gallery is represented by a single subject level feature computed for face, gait, and body using CAFace described in Sec. \ref{face-feature-encoding}, mean fusion on video-only gallery features, and mean fusion on whole body media excluding face-only imagery for each modality respectively. Many gallery images focus on the face only, and also the gait feature extraction method is not particularly well suited to single images, which motivates the exclusion of imagery for gait gallery features. For the body, the exclusion of the face-only images is done by thresholding the acceptable amount of vertical padding present in the preprocessed images, as face-only imagery will have body bounding box detections whose bounds extend far beyond the border of the image. Probe features are then compared to these gallery features, and equal-weighted score fusion is applied to generate a single score from the cosine similarity scores of the three modalities.

Due to the challenging conditions present in long-range, turbulent, and high-angle elevation imagery, it may sometimes be the case that feature extraction may not be successful for one or more modalities for a particular input media. To mitigate the negative impact of missing features and subsequently missing probe-gallery scores, we impute missing scores to the middle of the score metrics range, which is zero for the case of cosine similarity which is the similarity metric used to generate probe-gallery scores.

==> ref/sec_3_method_v2.tex <==


\section{FarSight: System Architecture}\label{sec:}

\subsection{Overview of FarSight}
% {\color{red} [Chris, MSU]}
%%
As shown in Fig.~\ref{fig:overview}, the FarSight system operates through an intricate assembly of six modules, each tailored for a specific function: detection and tracking, image restoration, three biometric modalities, namely, face, gait, and body feature extraction, and multi-modality fusion module. These modules function within a containerized testing framework, utilizing GPU resources effectively through dynamically adjustable batch sizes.

%%
An API utility bridges the interaction between the framework and external systems, streaming video sequences identified from configuration files to the testing framework using Google RPC calls. The framework then extracts vital features from these sequences, which are stored in HDF5 databases for match performance evaluation.


%%
The workflow begins with video sequence processing through the detection and tracking modules. Bounding box-detected images are cropped and dispatched to the gait and body feature encoding module. Simultaneously, the cropped face frames undergo image restoration before their delivery to the face module. 
%
Both the body and gait modules produce a unique per-sequence feature vector from a single run of all sequences via average pooling operation, while the face pipeline employs CAFace~\cite{caface} to aggregate the features across various sequences.

%The body and gait modules yield a singular per-sequence feature vector from a single pass of all sequences, while the face pipeline adopts CAFace to aggratee the features across features.

%a two-stage process. This process first produces intermediate AdaFace feature vectors for each frame, which are then refined by CAFace to generate the final feature vector.

%%
Catering to the varying needs of enrollments, the system processes probe enrollments as single video segments per subject, generating definitive feature vectors. Conversely, gallery enrollments, composed of multiple video sequences and still images, undergo additional consolidation, merging into a singular, comprehensive subject-level feature vector post-processing.

%\noindent 
%The FarSight system is comprised of five modules that provide functions for detection and tracking, image restoration, and the three biometric modalities: body extraction, face extraction and gait extraction.  Each module is wrapped in a standard interface and deployed in containerized testing framework.

%The testing framework listens for calls to standard functions for gallery and probe enrollment into a database, database manipulation functions for merging and finalizing, and scoring functions to generate raw matching data that can subsequently be processed to generate performance results.

%Calls to the testing framework originate via an API utility that takes configuration files that identify gallery and probe source media and streams media to the testing framework over Google RPC calls in a frame-by-frame manner.  Still images (gallery only) and videos (both gallery and probe) are submitted to the test framework for feature extraction and the framework writes extracted features out to databases in the HDF5 format. These databases can then be utilized to determine matching performance.

%Each module is executed asynchronously in its own process space, allowing for different batch sizes for each module to make best use of available GPU resources.  Results are synchronized at the end of processing of each media piece.

%Media is first sent to the detection and tracking modules and fed to subsequent modules, following appropriate pre-processing, as detection and tracking results become available.  Frame-by-frame image data and corresponding detection bounds are first pre-processed into appropriately cropped and scaled batches before sending to the body and gait modules.  Image restoration is applied to face frames before sending to the face module.  Both restored and unrestored imagery is sent to the face module to allow it to make a best-result judgement on which form to use.

%Body and gait both process all images in each discrete media in a single pass resulting in a single per-media feature vector respectively.  In contrast, the face pipeline processes in two stages, first generating intermediate AdaFace feature vectors for each frame in the source media, and then passing those intermediate feature vectors to CAFace to generate a resulting feature vector.

%Probe enrollments consist of a single video segment per subject, and thus the resulting feature vectors above are final.  Gallery enrollments, however, consist of multiple video and still images and the media-level feature vectors must be finalized into a single subject-level feature vector once all gallery media has been processed.
%Fig.~\ref{fig:overview} 


\begin{figure}[t]
\begin{center}
\includegraphics[width=0.95\linewidth]{fig/Feng/fig3_briar_examples.pdf}
\end{center}
   \caption{The examples in the BRIAR dataset~\cite{cornett2023expanding} illustrate the same subject under various conditions, including different distances, clothing, and varying image quality due to the turbulence effect. The columns represent different scenarios: controlled conditions, close range, 100m-set1, 100m-set2, 200m, 400m, 500m, and UAV respectively. The four subjects shown here (one per row) in the figure (ID: G02030, G02062, G02217 and G02229) consented to have their images included for publication.}
\label{fig:briar_examples}
\end{figure}

\subsection{Challenges in FarSight}
%{\color{red} [Feng, MSU]}

Our FarSight system faces an array of unique challenges.
%
Firstly, long-range capture and atmospheric turbulence often result in low-quality biometric samples that are difficult to process. Secondly, elevated platforms introduce large yaw and pitch angles, further complicating the data analysis. Additionally, the low visual quality hampers the extraction of identity information, making accurate recognition more difficult. The training data also presents a limitation, as its domain is restricted due to diverse environmental changes. Lastly, the low generalizability and explainability of deep learning models pose a significant challenge to the achievement of reliable and transparent results. 
%
In Fig.~\ref{fig:briar_examples}, we provide examples from close-range, mid-range (100m-500m), and UAV scenarios for a more visual understanding of these challenges. 

\subsection{Physics Modeling of Turbulence}

\noindent Atmospheric turbulence is an unavoidable degradation when imaging at range. It is often computationally modeled by splitting the continuous propagation paths into segments via phase screens as illustrated in Fig.~\ref{fig: turbulence simulation}. 
While accurate, the spatially varying nature of the propagation
%For \emph{every} point on the object plane, we need to perform a series of Fourier transforms and phase multiplications to compute the point spread function on the image plane \cite{Hardie_2017_a, Hardie_2022_a, Schmidt_2010_a}. 
makes this a computationally expensive process \cite{Hardie_2017_a, Hardie_2022_a, Schmidt_2010_a}.



\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{./fig/turbulence/turb_simulation}
\caption{Comparing split-step and Zernike-based simulations \cite{Chimitt_2020_a, Mao_2021_a, chimitt_2022_a}.}
\label{fig: turbulence simulation}
\end{figure}


More recent works have explored the possibility of \emph{propagation-free} models where the turbulence effects are implemented as random sampling at the \emph{aperture} \cite{Chimitt_2020_a, Mao_2021_a, chimitt_2022_a}. As shown in Fig.~\ref{fig: turbulence simulation}, every pixel on the aperture is associated with a random phase function which has a linear representation using the Zernike polynomials \cite{Noll_1976_a}. By constructing the covariance matrix of the random process, we can draw samples of the Zernike coefficients to enforce spatial and modal correlations. Propagation-free simulation has enabled $1000 \times $ speed up compared to the split-step propagation methods while maintaining the accuracy. Therefore, we adopt this simulation appraoch in our system.
%This will lead to two principal components of the turbulent effects: (1) tilt (i.e., geometric displacement of pixels) and (2) spatially varying blur \cite{Chan_2022_a},
% \begin{equation}
%     I(\mathbf{x}) = [\mathcal{B} \circ \mathcal{T}] (J(\mathbf{x})),
%     \label{eq: turb_img_form}
% \end{equation}
% where $\mathcal{T}$ is the tilt operator and $\mathcal{B}$ represents the blur operation, with $J(\mathbf{x})$ and $I(\mathbf{x})$ as the input and output images, indexed by position $\mathbf{x}$, respectively. 




For the generation of training data, realistic optical and turbulence parameters significantly influence the appearance of the generate defects. Therefore, our datasets are synthesized according to the metadata of various long-range optical systems. Our training dataset also consists of both dynamic and static scenes \cite{Safdarnejad_2015_a, Jin_2021_a, zhou2017places}. 


 %Solving the inverse problem of \eqref{eq: turb_img_form} is highly non-trivial and deviates from many classical deblurring problems \textcolor{red}{[a few citations]}, where blur is assumed to be uniform or the shifting to be global. 


% For learning-based restoration, imaging through turbulence poses a significant problem: ground truth is almost \emph{never} available -- if the image is observed through turbulence at one instance, we cannot ``turn it off'' in the next. Therefore, reliance on simulation for restoration is essential. Although existing methodologies exist \textcolor{red}{[split-step works]}, generating a sufficient amount of data is likely infeasible as noted by Chimitt et al. .
% %the generation a 4k dataset consisting of 1000 sequences with 100 frames each will take 156 years to process using split-step based methods.



%The series of works describing Zernike-based simulation  succeed in maintaining accuracy while increasing the speed by a factor of $\times\!1000$. Although the capability exists, proper selection of parameters and application to images in training is non-trivial. Improper application will overemphasize certain aspects such as pixel shifting or blur size, therefore, to accurately represent imaging through turbulence, we must choose the parameters carefully. Because we are specifically interested in biometric recognition, we can tailor our parameter choices for simulation to reasonably match our expectation for where our restoration may be applied. Exact parameter choices can be found in the supplementary document. The types of scenes we focus are fairly general, simulating on a few video datasets \cite{Safdarnejad_2015_a, Jin_2021_a, zhou2017places}.






\subsection{Detection and Tracking}
% {\color{green} [UO team]}
%%%% Will redo equations to avoid overflowing
%%%% Figures will be added soon.


Our detection module, based on Wan et al.'s method~\cite{wan2021bodyface}, uses a two-stage R-CNN detector~\cite{ren2015faster} with a modified ResNet50 backbone to associate face and body bounding boxes~\cite{wan2021bodyface}. This is done using associative embeddings to match faces and bodies, learned via \textbf{pulling} and \textbf{pushing} loss functions~\cite{}.

The pulling loss attempts to bring embeddings of the same subject closer, calculated as body-to-body, face-to-face, and face-to-body pairs. These are combined using a weighted sum of body-to-face loss, and the sum of face-to-face and body-to-body losses.
%
Pushing loss, in contrast, pushes away bounding boxes assigned to different subjects. It is divided into three losses between pairs of body boxes, pairs of face boxes, and body-face pairs. These losses are also combined via a weighted sum.
%
The final associative embedding loss used to optimize these embeddings is a weighted sum of the pulling and pushing losses.

The module also predicts "head hook" coordinates for every subject to improve body and face association. The head hook loss is a weighted sum of the Smooth L1 loss and a scale-invariant angular loss.

The final association between body and face bounding boxes is based on similarity metrics, including embedding distance, head hook distance, and confidence scores. The RBF kernel is used for both the embedding distance and head hook distance. The confidence scores factor directly into the association loss to mitigate associating low-confidence bounding boxes with high-confidence ones.

Finally, all these metrics are integrated into a final association metric. If a face prediction's maximum similarity score with any body is below a set threshold, it is concluded that the subject's face is not visible.










\subsection{Image Restoration} 

Image restoration aims to reverse the image formation process, as described by the equation~\cite{Chan_2022_a}
\begin{equation}
    I(\mathbf{x}) = [\mathcal{B} \circ \mathcal{T}] (J(\mathbf{x})),
    \label{eq: turb_img_form}
\end{equation}
where $\mathcal{T}$ is the tilt operator and $\mathcal{B}$ represents the blur operation, with $J(\mathbf{x})$ and $I(\mathbf{x})$ as the input and output images, indexed by position $\mathbf{x}$, respectively. In this work, we have considered a single-frame image restoration method as well as a multi-frame method, both aiming to invert $\mathcal{T}$ and $\mathcal{B}$. 


Our restoration methods for biometrics focus on preserving identity, using lightweight, real-time techniques. These are divided into single-frame and multi-frame restorations. The former provides lower throughput but relies on strong priors without altering the subject's identity. Multi-frame restoration, on the other hand, utilizes temporal information, allowing weaker priors but requiring larger throughput.


Our multi-frame approach uses the Recurrent Turbulence Mitigation network (RTM), a bi-directional, multi-scale convolutional recurrent network with an innovative Multi-head Temporal Channel self-attention (MTCSA) layer (Fig. \ref{fig: rtm}).
%
For single-frame restoration, we employ Mao et al~\cite{Mao_2022_a}.'s Turbulence Mitigation Network (TurbNet), which estimates turbulence distortion during restoration (Fig. \ref{fig: TurbNet}). After restoration, the estimate is re-distorted for prediction evaluation.


\begin{figure}[h]
    \centering
    \includegraphics[width = 0.9\linewidth]{fig/turbulence/RTM_simple.jpg}
    \caption{Multi-frame image restoration by the recurrent network for turbulence mitigation (RTM).}
    \label{fig: rtm}
\vspace{-3ex}
\end{figure}


\begin{figure}[h]
    \centering
    \includegraphics[width = \linewidth]{fig/turbulence/main_arch_eccv}
    \caption{single-frame image restoration by TurbNet.}
    \label{fig: TurbNet}
\vspace{-3ex}
\end{figure}












\subsection{Multi-Modal Biometric Feature Encoding} %{\color{red} [Ryan and Feng, MSU]}}

We describe here our methods for obtaining identifying biometric features from our face, gait and body matching modules, as well as the multi-modal fusion technique applied to generate fused scores for evaluation on the various metrics described in Sec. \ref{evaluation-metrics}.

\subsubsection{Face }
\label{face-feature-encoding}
%{\color{green} [Minchul, MSU]}

Herein, we describe our face recognition pipeline that incorporates the methods of AdaFace~\cite{kim2022adaface}, CAFace~\cite{caface}, and CFSM~\cite{liu2022cfsm}, creating a comprehensive approach to overcome the challenges of recognizing faces across varied image qualities with both image and video media.

Our pipeline initiates with AdaFace~\cite{kim2022adaface}, an adaptive loss function technique designed for handling low-quality face datasets. The framework uses image quality to adaptively modulate the emphasis on misclassified samples, a feature particularly effective for managing the wide range of image qualities.

Further enhancement of our pipeline involves the implementation of CAFace~\cite{caface}, a two-stage feature fusion paradigm that is indispensable for incorporating features across multiple frames. By assigning inputs to a limited number of global cluster centers and later fusing the clustered features, CAFace provides the ability to combine multiple frames while maintaining order invariance.

Lastly, our pipeline incorporates the Controllable Face Synthesis Model (CFSM)~\cite{liu2022cfsm}. Given the persistent challenge of domain gaps between semi-constrained training datasets and unconstrained testing scenarios, CFSM provides a solution by mimicking the target datasets' distribution in a style latent space. This face synthesis model allows for precise control over the diversity and degree of synthesis, and the pre-trained synthesis model is designed to be guided by the FR model, generating images that are more beneficial for FR model training. Crucially, this approach allows us to generate synthetic face images similar in style to the target evaluation datasets, bridging the gap between high-quality training data and lower-quality surveillance images.

The amalgamation of AdaFace, CAFace, and CFSM within our pipeline forms a comprehensive solution to the challenges of face recognition across a diverse range of image qualities. Through effective frame-level feature extraction, integration of these features, and controllable synthetic image generation, our approach achieves substantial improvements in face recognition tasks across both high and low-quality image datasets.

\subsubsection{Gait }
%{\color{red} [Yiyang, MSU]}

Gait recognition is a biometric technique that focuses on analyzing an individual's walking patterns and movements to identify and differentiate them from others. 
% Unlike other biometric modalities like facial recognition, gait patterns can be captured from a distance and/or altitude.
It is particularly advantageous for long-distance and high-altitude surveillance applications, such as surveillance cameras mounted on buildings and unmanned aerial vehicles (UAVs), due to its ability to capture and analyze gait patterns from a distance. 
Unlike other biometric modalities like facial recognition, gait recognition can work effectively even when the subject's face is obscured, making it valuable in long-range and aerial scenarios. 
Additionally, gait recognition takes advantage of the dynamic nature of walking, capturing the unique rhythm, pace, and motion characteristics exhibited by individuals while other biometric modalities such as face recognition and body matching primarily rely on static features.
Focusing on the inherent temporal cues of gait enhances the accuracy and reliability of biometric identification in scenarios where other modalities may fall short.

Through our observations, we have identified a limitation in the current state-of-the-art gait recognition models, specifically their predominant focus on extracting local gait features while neglecting the essential global correlations. These global correlations refer to the interdependencies between different body parts across various frames of a gait sequence. In order to address this limitation and enhance the discriminability of gait recognition, we propose an innovative framework named GlobalGait. This framework aims to enrich the local gait features by incorporating and leveraging the crucial global correlations, thereby improving the overall effectiveness and accuracy of gait recognition.

In particular, given an input sequence \(\left(\mathbf{I}_1, \mathbf{I}_2, \dots, \mathbf{I}_{N}\right)\), we first use a CNN backbone to extract local spatiotemporal features \(\mathbf{F}_{\mathit{backbone}}\), which is then divided into \(\mathbf{F}_{\mathit{source}}\) and \(\mathbf{F}_{\mathit{target}}\). 
We project the feature maps to tokens \(\mathbf{T}\) for each joint by sampling around each 2D joint. 
And then, we use a stack of multi-head self-attention layers to model the spatial and temporal correlations in the sequences. 

To provide additional supervision signals for mining global correlations, we instruct our model to reconstruct the target frame pixels based on source sequences and select the correct target sequence among a batch of candidates. 
The goal is to exploit the spatial and temporal correlations in gait recognition and have these supervision signals provide feedback so that the model can learn more discriminative gait features.


\subsubsection{Body}
% {\color{red} [Feng, MSU]}
%%
The body feature encoding is an essential element of identity representation, widely used in person re-identification (Re-ID), search and tracking. In this subtask, we will leverage the Re-ID search to effectively encode the static body features.
%
Person Re-ID aims to re-identify a query person from a large image collection, taken by multiple cameras at different times~\cite{ye2021deep,ahmed2015improved,zheng2015scalable,li2018harmonious}. 
%
It is challenging due to the geometric misalignment and appearance ambiguity caused by the diversity of human poses and their clothing.
Thus, it is crucial to develop effective solutions to extract static body features that are robust to body pose and cloth-changing variations. 


%%
To address these challenges, we posit that the most reliable cue for body matching is the $3$D naked (unclothed) body shape, if it can be accurately and discriminately estimated from a $2$D body image.
%
The challenge of reconstructing a $3$D naked body is significant due to confounding factors and the lack of supervision, such as paired images and $3$D naked body scans. However, taking inspiration from recent advancements in $3$D feature learning for face recognition~\cite{peng2017reconstruction,liu2018disentangling}, we propose a novel pipeline to disentangle identity (naked body) from non-identity components (pose, clothing shape and texture) of $3$D clothed humans. 


%%%%%%% ----------- Figure ------------  %%%%%%%%%%
\begin{figure}[t]
  \centering
  \includegraphics[width=1\linewidth]{fig/Feng/bm_flowchart.pdf}
   \caption{\small Overview of the proposed body feature encoding framework. In the body matching process, the identity shape features $\mathbf{z}_{id}$ is utilized for matching.}
   \label{fig:bm_flowchart}
   %\vspace{-2mm}
\end{figure}
%%%%%%% ----------- Figure ------------  %%%%%%%%%%

%%
In particular, as illustrated in Fig.~\ref{fig:bm_flowchart}, the proposed method relies on a new joint two-layer neural implicit function that represents $3$D humans, where identity, clothing shape, and texture components are represented in disentangled latent representations.
%
Formally, given a training set of $T$ images $\{\mathbf{I}_i\}_{i=1}^{T}$ and the corresponding identity labels $\{l_i\}_{i=1}^{T}$,
the image encoder $\mathcal{E}(\mathbf{I}):\mathbf{I}\xrightarrow{} \mathbf{z}_{id}, \mathbf{z}_{cloth}, \mathbf{z}_{tex}$ predicts the identity shape code of naked body $\mathbf{z}_{id}\in\mathbb{R}^{L_{id}}$, clothed shape code $\mathbf{z}_{cloth}\in\mathbb{R}^{L_{cloth}}$ and texture code $\mathbf{z}_{tex}\in\mathbb{R}^{L_{tex}}$. A joint two-layer implicit model decodes the latent codes to identity shape, clothing shape, and texture components, respectively. 
%
Additionally, PoseNet $\mathcal{P}$ predicts the camera projection $\mathbf{\Omega}$ and SMPL body pose $\mathbf{\theta}$: $(\mathbf{\Omega}, \mathbf{\theta}) = \mathcal{P}(\mathbf{I})$.
%
Mathematically, the learning objective is defined as:
\begin{equation}
\label{eqn:objective}
\argmin_{\mathcal{E},\mathcal{F},\mathcal{C},\mathcal{T}} \sum_{i=1}^T \left(\left|\hat{\mathbf{I}}_i -  \mathbf{I}_i\right|_1 
+ \mathcal{L}_{cla}(\mathbf{z}_{id},l_i)\right),
\end{equation}
where $\mathcal{L}_{cla}$ is the classification loss. $\hat{\mathbf{I}}$ is the rendered image.
%
This  objective enables us to jointly learn accurate $3$D clothed shape and discriminative shape for the naked body.

%%
We employ a combination of CAPE~\cite{ma2020learning} and THuman2.0~\cite{zheng2019deephuman} datasets to instruct our joint two-layer implicit model. Each scan is processed to yield SMPL naked shape code and joint locations. Each training sample is assigned its own identity shape code, clothing shape code, and texture code through autodecoding.
%
For inference, the encoder $\mathcal{E}$ processes body images and extracts the identity shape features $\mathbf{z}_{id}$. The Cosine similarity of $\mathbf{z}_{id}$ is then used to determine if the two images belong to the same person. It is worth noting that, as the $3$D reconstruction module is not involved in this inference, it is highly efficient.

\subsubsection{Multi-Modality Fusion}
% {\color{red} [Ryan]}

To generate a probe-gallery score from multiple biometric modalities, first per modality scores are computed for all probe-gallery pairs. Each Gallery is represented by a single subject level feature computed for face, gait, and body using CAFace described in Sec. \ref{face-feature-encoding}, mean fusion on video-only gallery features, and mean fusion on whole body media excluding face-only imagery for each modality respectively. Many gallery images focus on the face only, and also the gait feature extraction method is not particularly well suited to single images, which motivates the exclusion of imagery for gait gallery features. For the body, the exclusion of the face-only images is done by thresholding the acceptable amount of vertical padding present in the preprocessed images, as face-only imagery will have body bounding box detections whose bounds extend far beyond the border of the image. Probe features are then compared to these gallery features, and equal-weighted score fusion is applied to generate a single score from the cosine similarity scores of the three modalities.

Due to the challenging conditions present in long-range, turbulent, and high-angle elevation imagery, it may sometimes be the case that feature extraction may not be successful for one or more modalities for a particular input media. To mitigate the negative impact of missing features and subsequently missing probe-gallery scores, we impute missing scores to the middle of the score metrics range, which is zero for the case of cosine similarity which is the similarity metric used to generate probe-gallery scores.

==> ref/sec_4_exp_v1.tex <==


\begin{table*}[t]
    \centering
\resizebox{0.98\linewidth}{!}{
    \begin{tabular}{|c||p{1.8cm}<{\centering}|p{1.8cm}<{\centering}|p{1.8cm}<{\centering}||p{1.8cm}<{\centering}|p{1.8cm}<{\centering}||p{1.8cm}<{\centering}|p{1.8cm}<{\centering}|}
     \hline
      \multirow{2}{*}{Method} & \multicolumn{3}{c||}{ \makecell{\textbf{Verification (1:1)} \\ TAR@1\%FAR $\uparrow$} } & \multicolumn{2}{c||}{\makecell{\textbf{Rank Retrieval (1:N)} \\ Top20, Closed Search  $\uparrow$}}  & \multicolumn{2}{c|}{\makecell{\textbf{Open Search (1:N)} \\ FNIR @ 1\%FPIR$\downarrow$} } \\
      \cline{2-8}
      & $\textup{Whole Body}^{1}$ & $\textup{Whole Body}^{2}$ & Face Only & Whole Body & Face Only &  Whole Body & Face Only \\ 
      
     \hline\hline
 Baseline-AdaFace~\cite{kim2022adaface}     & 
 %24.95
 - & -- & 66.20 & -- & 73.85 & -- & 70.64 \\       
 \textbf{FarSight-Face}    & 
 %25.04 
 - & -- & 78.01 & -- & 84.12 & --  & 57.39\\       
 Baseline-GaitBase~\cite{gaitbase}    & 44.33 & 45.55 & -- & 62.60 & -- & 98.38 & -- \\       
 \textbf{FarSight-Gait}    & ??.?? & ??.?? & -- & ??.?? & -- & ??.??  & -- \\       
 Baseline-CAL~\cite{CAL}         & 48.58 & 51.87 & -- & 51.87 & -- & 96.17 & -- \\       
 \textbf{FarSight-Body}    & 51.02 & 54.00 & -- & 72.91 & -- & 96.23 & -- \\    
 \hline \hline
  Baseline     & 59.8 & 80.30 & 66.20 & 31.89 & 73.85 & 100 & 70.64\\
 \textbf{FarSight-Face+Gait}     & 45.51 & 83.41 & -- & 30.65 & -- & 100 & --\\
\textbf{FarSight-Face+Body}     & 43.95 & 85.84 & -- & 92.73 & -- & 58.99 & -- \\ 
 \textbf{FarSight-Gait+Body}     & 58.91 & 62.08 & -- & 27.46 & -- & 100 & --\\
 \textbf{FarSight}     & ??.?? & ??.?? & 78.01 & ??.?? & 84.12 & ??.?? & 57.39\\
 \hline
    \end{tabular}
    }
        \caption{Whole body biometric recognition results on the BRIAR dataset.}
	\label{tab:bts_results}
\end{table*}


\begin{table}[t]
    \centering
\resizebox{0.98\linewidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|}
     \hline
     Probe & Close range & 100m & 200m & 400m & 500m & UAV & Mean\\ 
     \hline\hline
 \textbf{FarSight-Face}    & ?? & ?? & ?? & ?? & ?? & ??  & ??\\       
 \textbf{FarSight-Gait}    & ?? & ?? & ?? & ?? & ?? & ??  & ??\\       
 \textbf{FarSight-Body}    & ?? & ?? & ?? & ?? & ?? & ?? & ??\\    
 \textbf{FarSight}     & ?? & ?? & ?? & ?? & ?? & ?? & ??\\
 \hline
    \end{tabular}
    }
        \caption{Rank-20 accuracy (\%) on BRIAR at different altitudes and ranges.}
	\label{tab:bts_distance_results}
\end{table}


\section{Experimental Results}\label{sec:exp} 

% BRIAR dataset paper https://openaccess.thecvf.com/content/WACV2023W/LRR/papers/Cornett_Expanding_Accurate_Person_Recognition_to_New_Altitudes_and_Ranges_The_WACVW_2023_paper.pdf

%{\color{red} All results should be obtained from our container using the BRIAR dataset (BGC1 + BGC2).}



\subsection{Setting }
%  {\color{red} [ MSU]}

All modules are run together in a configurable container environment using PyTorch version 1.13.1. Experiments are performed using 8 NVIDIA RTX A6000s, having 48 GiB of VRAM, over the course of 48 hours on 2 dual socket servers with either AMD EPYC 7713 64-Core or Intel Xeon Silver 4314 32-Core processors.

\Paragraph{BRIAR Datasets and Protocols.}
%   {\color{red} [Feng, MSU]}
%
The BRIAR dataset~\cite{cornett2023expanding}, comprised of two major collections— BRIAR Government Collections 1 (BGC1) and 2 (BGC2), is a pioneering initiative to support whole-body biometric recognition research. It addresses the necessity for broader and richer data repositories for training and evaluating biometric systems for challenging applications. Utilizing an array of imaging components, including DSLR cameras, surveillance systems, and UAV platforms, BRIAR consists of over $350,000$ images and $1,300$ hours of video footage from $1,055$ distinct subjects in outdoor settings.
%
The BRIAR dataset, with its focus on long-range and elevated angle recognition, provides a fertile ground for algorithm development and evaluation, contributing to significant strides in whole-body recognition research.

The dataset has been partitioned into a training subset (BRS) and a testing subset (BTS) according to the provided Protocol V2.0.1. 
% 
For evaluation purposes, the probe sets have been categorized into two distinct groups: FaceIncluded and FaceRestricted. 
%
The FaceIncluded set comprises data where the face of the subjects is clearly visible, occupying a minimum of 20 pixels in head height, with the width potentially varying due to changes in the yaw angle of the head. 
%
On the other hand, the FaceRestricted set consists of data that presents challenges such as occlusion, low resolution, or unusable faces. 
%
These sets have been further subdivided into treatment and control sets to facilitate focused analysis. The experimental control subset consists of cameras positioned at close range, typically within 75 meters. 
%
These cameras are primarily used to establish performance expectations based on traditional methods. 
% It is worth noting that most close-range cameras possess wide fields of view to capture the entire walking area, which may result in lower resolution, potentially impacting the accuracy of face recognition. 
Conversely, the treatment sets comprise cameras situated at long distances or elevated angles, as well as UAVs. 
These configurations are of primary interest as they simulate real-world surveillance scenarios and pose specific challenges for biometrics.
% The main objective of this protocol is to delineate probe templates that emulate the desired conditions, by defining two categories of probes: \emph{control} and \emph{treatment}. The control category encompasses BGC videos where the subject's face or body can be easily recognized. The performance of this protocol provides a benchmark indicating an optimal functioning scenario for biometric recognition. Conversely, the treatment category consists of video clips where the recognition of the subject's face or body poses a greater challenge. The performance under the treatment setting serves as a gauge for the target scenario of the BRIAR evaluation.

%%
\Paragraph{Evaluation Metrics. }
\label{evaluation-metrics}
% {\color{green} [Minchul, MSU]}
We employ BRIAR Program Target Metrics~\cite{bba} to measure the FarSight system's performance across multiple modalities and their fusion: 
%
(i) verification (TAR@1\%FAR), (ii) closed-set identification (Rank-20 accuracy), and (iii) open-set identification (FNIR@1\%FPIR), allowing for a thorough examination of its performance across various conditions. 
%
Moreover, the system is evaluated in two modes -- face only and whole body.


%Verification is a task that assesses whether two given media, which can be images or videos, represent the same subject. In terms of performance metrics, one common measure is the Area Under the Curve (AUC) of match scores. AUC is a reliable indicator of the effectiveness of the verification system; a higher AUC (close to $1.0$) represents better separation between matches and non-matches. Additionally, to understand the performance at a specific operating point, True Acceptance Rate at a particular False Acceptance Rate (TAR@FAR) is often employed. In our discussions, we will use TAR@1\%FAR as an indicator of performance at a specific threshold.

%Identification is a task that involves recognizing an unknown individual (probe) from a known database (gallery). This task can be further divided into closed-set and open-set scenarios. In the closed-set scenario, all potential probe subjects are guaranteed to be present in the gallery. On the contrary, in the open-set scenario, the probe subjects may or may not be present in the gallery.

%For closed-set identification, the performance is usually measured by Rank-N accuracy. It is because closed-set search, alternatively known as Rank Retrieval, refers to an identification task where each probe has a corresponding match within the gallery of templates. In this scenario, given a probe video, the executing algorithm is tasked with returning the top R gallery matches that are associated with the probe.
%For instance, Rank-20 accuracy indicates how often the true match for a probe template is within the top 20 closest gallery templates. 

%The performance of a closed-set search can also be  quantified by the True Positive Identification Rate (TPIR) — representing the frequency at which the algorithm accurately retrieves a match for a probed template — and the False Negative Identification Rate (FNIR), which denotes the frequency of erroneous no-match returns by the algorithm for a probed template. A Cumulative Match Characteristic (CMC) curve, derived from these TPIR and FNIR values, succinctly encapsulates an identification algorithm's accuracy in matching search results and its proficiency in ranking the gallery results based on similarity.

%For open-set identification, performance is typically measured by the False Negative Identification Rate at a specific False Positive Identification Rate (FNIR@FPIR), specifically FNIR@1\%FPIR in our case.

%Through these metrics, we aim to assess the performance of our recognition pipeline across a variety of conditions and modalities including face, body, and gait. The corresponding performances will be summarized in the following sections.

\Paragraph{Baselines.}
%[{\color{green} Minchul \color{red} Ryan, Yiyang and Feng, MSU]}
%
In our study, we utilize established benchmarks for each biometric modality to ensure a comprehensive comparison: For facial recognition, we utilized AdaFace coupled with an average feature aggregation strategy, a popular approach known for its excellent performance~\cite{kim2022adaface}. For gait recognition, we adopted GaitBase~\cite{gaitbase}, a solution known for its efficacy. For body modality, we employed CAL~\cite{CAL}, a SoTA cloth-changing person re-identification method. These benchmarks provide an excellent basis to fairly evaluate our proposed method.

%In Tab.~\ref{tab:bts_results}, we provide the benchmark performance of publically available methods.  For the face modality, we use ArcFace~\cite{arcface} with the average feature aggregation as a benchmark. 
%For the gait modality, we use GaitBase~\cite{gaitbase} as our baseline. For the body modality, we use CAL~\cite{CAL}, SoTA Cloth-changing person re-identification method as our baselines.

\subsection{Evaluation and Analysis}

%{\color{red} Conducting Ablation Studies: Evaluating the Impact of Image Restoration and Detection on Biometric Recognition}

%We conduct an extensive comparison between our approaches and the baselines for each modality in Tab.~\ref{tab:bts_results}.
% 
%The detailed side-by-side analysis offers a clear perspective on our approaches' performance compared to the baselines.

In Tab.~\ref{tab:bts_results}, we provide a thorough comparison of our approaches and the baselines for each modality. The detailed comparison analysis clearly highlights the superior performance of our proposed FarSight system across all performance metrics when compared to the baselines.
%
We further investigate and report on the Rank-20 accuracy using the BRIAR dataset, taking into consideration differing altitudes and ranges. 
%
As illustrated in Tab.~\ref{tab:bts_distance_results}, ....

\subsubsection{Face}
% {\color{red} [Minchul, MSU]}
The efficacy of including various modules in the face recognition pipeline is shown in Tab.~\ref{tabl:faceparts}. We initially used the combination of AdaFace IR101 backbone with the average feature aggregation which has shown good performance in low quality imageries~\cite{kim2022adaface}.  CFSM~\cite{liu2022cfsm} adds performance improvement by adopting training data to a low-quality image dataset WiderFace~\cite{widerface} ($+1.18$ in TAR@1\%FAR). CAFace~\cite{caface} is a feature fusion method which improves upon the basic average pooling (+$4.16$). Lastly, finetuning the model on the BGC1 training dataset further improves the performance (+$6.47$).  

The addition of image restoration using RTM based restoration model is shown in Tab~\ref{tabl:facerestore}. The performance improvement is observed in the challenging \textit{face included treatment} group. However, for the easy \textit{face included control} group, the restoration is not helpful. 


\begin{table}[!ht]
    \centering
    \small
    \begin{tabular}{|c|c|c|c|}
    \hline
       Face Inc.Treatment & \makecell{TAR@\\1\%FAR} & \makecell{Rank\\20} & \makecell{FNIR@\\1\%FPIR} \\ \hline
        AdaFace~\cite{kim2022adaface} & $66.20$ & $73.85$ & $70.64$ \\ \hline
         + CFSM~\cite{liu2022cfsm} & $67.38$ & $77.22$ & $68.51$ \\ \hline
         + CAFace~\cite{caface} & $71.54$ & $78.57$ & $61.77$ \\ \hline
        \makecell{+BRS1 \\(FarSight-Face) }  &  $78.01$	& $84.12$	 & $57.39$   \\ \hline
        % \makecell{+Aligner} &  &  &  \\ \hline
    \end{tabular}
    \caption{Ablation of different parts in face recognition pipeline. }
    \label{tabl:faceparts}
\end{table}



\begin{table}[!ht]
    \centering
    \small
    \begin{tabular}{|r|c|c|c|}
    \hline
       TAR@1\%FAR & \makecell{Face Inc.\\Control} & \makecell{Face Inc.\\Treatment} & \makecell{Face Inc.\\All} \\ \hline
        Face + Restoration & $\mathbf{96.03}$ & $72.39$ & $77.70$ \\ \hline
        Face - Restoration & $95.79$ & $\mathbf{72.57}$ & $\mathbf{77.81}$ \\ \hline
        % \makecell{+Aligner} &  &  &  \\ \hline
    \end{tabular}
    \caption{Face recognition with and without image restoration.}
    \label{tabl:facerestore}
\end{table}

%-------------------------------------------------------%
\subsubsection{Gait}
% {\color{red} [Ryan and Yiyang, MSU]}
% \paragraph{FarSight-Gait vs. GaitBase~\cite{gaitbase}.}
In our gait recognition experiments, we observed consistent improvements compared to GaitBase~\cite{gaitbase}, our baseline, across all four metrics.
%
Our findings demonstrate significant enhancements in the model's ability to accurately verify individuals, with the TAR@1\%FAR reaching an impressive improvement of \(xx.xx\%\) in WB\(^1\) and \(yy.yy\%\) in WB\(^2\). 
%
Furthermore, the top-20 rank retrieval metric exhibited notable advancement, showcasing a remarkable increase of \(zz.zz\%\) compared to our baseline. 
%
Lastly, our model showcased improved performance in open-set search, achieving a noteworthy reduction of \(ww.ww\%\) in FNIR@1\%FPIR.
%
These promising outcomes reaffirm the efficacy of FarSight-Gait to extract more discriminative features based on global features and highlight its potential for reliable and robust biometric identification in real-world applications.

%-------------------------------------------------------%
\subsubsection{Body}
% {\color{red} [Feng, MSU]}
\noindent\emph{Body matching vs. Gait recognition.} The performance of body matching and gait recognition varies depending on conditions. As shown in Tab.~\ref{tab:bm_mission_results_comparison}, gait recognition outperforms body in turbulent, low-resolution situations, thanks to its resilience. On the other hand, body matching excels in elevated views, where the 3D body shape can still be deduced even when gait becomes less distinguishable.

\noindent\emph{Body Matching Observations.}
In Fig.~\ref{fig:body_matching_paired_examples}, we show succeeded and failed matches in body matching. Our method copes well with clothing differences, but struggles with motion blur, turbulence, or hairstyle changes. Misidentifications in impostor pairs often happen due to similar body shapes.

\begin{table}[t!]
\small

\centering
\resizebox{0.98\linewidth}{!}{
\begin{tabular}{|l|c|c|c|c|c|}
\hline 
Protocol     &Metric      & \textbf{FarSight-Gait}   & \textbf{FarSight-Body}  \\
\hline 
LR Turbulence   & \multirow{2}{*}{Rank20 $\uparrow$}  &  $\textbf{??.??}$ & $??.??$ \\
Elevated        &   &  $??.??$ & $\textbf{??.??}$ \\
\hline 
    LR Turbulence   &  \multirow{2}{*}{TAR@1\%FAR $\uparrow$} & $\textbf{??.??}$ & $??.??$ \\
Elevated        &   & $??.??$ & $\textbf{??.??}$      \\
%\hline\hline
%LR Turbulence   &  \multirow{2}{*}{ FNIR@1\%FPIR} & $98.41$   & %$\textbf{97.95}$ \\
%Elevated        & & $96.97$   & $\textbf{96.05}$    \\
\hline
\end{tabular}
}
\caption{Comparison between body matching and gait recognition on Mission LR Turbulence and Elevated: the two missions where neither modality has the most advantage.}
\label{tab:bm_mission_results_comparison}
\end{table}

\begin{figure}[t!]
\begin{center}
\resizebox{1\linewidth}{!}{
\begin{tabular}{c c c c c}
{\includegraphics[height=3cm]
{fig/Feng/pairs/hs_genuine/BTS1.0_G00003_field_0000114712____BTS1_G00003_controlled_0000002844____1.0601.png}} & 
{\includegraphics[height=3cm]{fig/Feng/pairs/hs_genuine/BTS1.0_G00071_field_0000118399____BTS1_G00071_controlled_0000002938____1.143.png}} &
{\includegraphics[height=3cm]{fig/Feng/pairs/hs_genuine/BTS1.0_G00073_field_0000119810____BTS1_G00073_controlled_0000001413____1.1114.png}} &
{\includegraphics[height=3cm]{fig/Feng/pairs/hs_genuine/BTS1.0_G00293_field_0000136963____BTS1_G00293_controlled_0000004716____1.0602.png}} &
{\includegraphics[height=3cm]{fig/Feng/pairs/hs_genuine/BTS1.0_G00448_field_0000157658____BTS1_G00448_controlled_0000005519____1.1014.png}}  \\
\multicolumn{5}{c}{\LARGE (a) Successful Recognition of Genuine Pairs}\vspace{3mm}\\ 
{\includegraphics[height=3cm]{fig/Feng/pairs/ls_impostor/BTS1.0_G00083_field_0000121633____BTS2_G02678_controlled_0000041763____-0.60766.png}} & 
{\includegraphics[height=3cm]{fig/Feng/pairs/ls_impostor/BTS1.0_G00246_field_0000130545____BTS2_G02529_controlled_0000032686____-0.64466.png}} &
{\includegraphics[height=3cm]{fig/Feng/pairs/ls_impostor/BTS1.0_G00380_field_0000150022____BTS2_G02682_controlled_0000042160____-0.61029.png}} &
{\includegraphics[height=3cm]{fig/Feng/pairs/ls_impostor/BTS2.0_G02005_field_0000551568____BTS1_G00143_controlled_0000005168____-0.61122.png}} &
{\includegraphics[height=3cm]{fig/Feng/pairs/ls_impostor/BTS2.0_G02053_field_0000578230____BTS1_G00236_controlled_0000007772____-0.60312.png}}  \\
\multicolumn{5}{c}{\LARGE (b) Successful Recognition of Impostor Pairs}\vspace{3mm}\\
{\includegraphics[height=3cm]{fig/Feng/pairs/ls_genuine/BTS1.0_G00026_field_0000116303____BTS1_G00026_controlled_0000003233____-0.038741.png}} & 
{\includegraphics[height=3cm]{fig/Feng/pairs/ls_genuine/BTS1.0_G00162_field_0000123789____BTS1_G00162_controlled_0000012232____0.17941.png}} &
{\includegraphics[height=3cm]{fig/Feng/pairs/ls_genuine/BTS2.0_G02011_field_0000552533____BTS2_G02011_controlled_0000013408____0.20464.png}} &
{\includegraphics[height=3cm]{fig/Feng/pairs/ls_genuine/BTS2.0_G02052_field_0000575654____BTS2_G02052_controlled_0000007329____0.16695.png}} &
{\includegraphics[height=3cm]{fig/Feng/pairs/ls_genuine/BTS2.0_G02063_field_0000582889____BTS2_G02063_controlled_0000000524____0.17496.png}}  \\
\multicolumn{5}{c}{\LARGE (c) Failure Cases for Genuine Pairs}\vspace{3mm}\\
{\includegraphics[height=3cm]{fig/Feng/pairs/hs_impostor/BTS1.0_G00003_field_0000114924____BTS1_G00044_controlled_0000001130____1.0442.png}} & 
{\includegraphics[height=3cm]{fig/Feng/pairs/hs_impostor/BTS1.0_G00134_field_0000122985____BTS1_G00071_controlled_0000002938____1.0872.png}} &
{\includegraphics[height=3cm]{fig/Feng/pairs/hs_impostor/BTS1.0_G00286_field_0000136103____BTS1_G00124_controlled_0000004193____1.0882.png}} &
{\includegraphics[height=3cm]{fig/Feng/pairs/hs_impostor/BTS1.0_G00469_field_0000160417____BTS1_G00393_controlled_0000017635____1.0609.png}} &
{\includegraphics[height=3cm]{fig/Feng/pairs/hs_impostor/BTS1.0_G00550_field_0000169999____BTS1_G00304_controlled_0000008032____1.0825.png}}  \\
\multicolumn{5}{c}{\LARGE (d) Failure Cases for Impostor Pairs}\\
\end{tabular}
}
\end{center}
\vspace{-3mm}
\caption[\small Examples of successful recognition and failure cases of genuine and impostor pairs in body matching.]{\small Examples of successful/failed genuine and impostor pairs in body matching.
} 
\label{fig:body_matching_paired_examples}
\end{figure}

%-------------------------------------------------------%
%\subsubsection{Multi-Modality Fusion}
\subsubsection{Multi-Modal Fusion}
% {\color{red} [Ryan, MSU]}

\subsubsection{System Efficiency}
%{\color{red} [Chris, MSU]}
 
%Feature vectors for face, gait and body are of sizes 512, 7936 and 6144. Multiplying these values by 8 and dividing by 128 provides us with the template sizes: $4$KB, $62$KB and $48$KB, respectively. and $114KB
%\begin{table}
%    \centering
%    \begin{tabular}{|c|c|c||c|}\hline
%                      Body & Face & Gait & Combined \\\hline
%       $48$ & $4$ & $62$ & $114$\\\hline
%    \end{tabular}
%    \caption[Template sizes.]{Template sizes (KB).}
%    \label{tab:size}
%\end{table}
%
\paragraph{Template sizes.} Feature vectors for face, gait and body are of sizes $512$, $7936$ and $6144$. Multiplying these values by 8 and dividing by 128 provides us with the template sizes: $4$KB, $62$KB and $48$KB, respectively, and $114$KB in total.

%
\paragraph{Processing speed.} The speed of our FarSight system, as outlined in Tables~\ref{tab:processing_time}, is examined under stringent conditions to gauge both the efficiency of individual components and the overall pipeline. This system operates asynchronously and concurrently, similar to the actual deployment conditions. For the sake of precise efficiency measurements, the components were assessed in a serialized manner, even though they typically run in parallel.
%
We conducted this assessment using representative sample videos, encompassing 2400 frames of 1080p and 1200 frames of 4k video, each set originating from four distinct subjects. The restoration process is primarily directed towards detected faces, which implies that any instances of undetected faces would naturally lead to reduced restoration and face module processing times. A notable observation is that our system can successfully detect bodies in 95\% of all frames and faces in 26\% of frames.

%Processing speed statistics are displayed in Tables~\ref{tab:processing_time} and ~\ref{tab:speed_pipeline}. Module components run asynchronously and concurrently in the deployed pipeline. To isolate component efficiency, an evaluation is executed by processing pipeline components serially rather than concurrently.  Individual component efficiency is displayed in seconds and overall pipeline performance is represented in frames per second (fps).


\begin{table}
    \centering
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{|c|c|c|c|}\hline
        Module & 1080p & 4K & Average Combined\\ \hline \hline
        Detection \& Tracking & $20.0$ & $34.7$ & $24.9$ \\ \hline
        Restoration           & $6.1$  & $5.3$  & $5.9$\\ \hline
        Face                  & $2.6$  & $2.2$  & $2.5$\\ \hline
        Gait                  & $3.3$  & $2.5$  & $3.0$\\ \hline
        Body                  & $3.7$  & $3.1$  & $3.5$\\ \hline \hline
        Speed (fps) & $8.4$ & $6.3$ &  $7.8$\\ \hline
    \end{tabular}
    }
    \caption{Processing time and average speed of each FarSight system module.}
    \label{tab:processing_time}
    \vspace{-2mm}
\end{table}

%\begin{table}
%    \centering
%    \begin{tabular}{|c|c|c|c|}\hline
%        Media              & 1080p & 4K & Average Combined \\ \hline
%        Speed (fps) & $8.4$ & $6.3$ &  $7.8$\\ \hline
%    \end{tabular}
%    \caption{Average Speed of Frame Processing in our FarSight.}
%    \label{tab:speed_pipeline}
%\end{table}

%Sample videos that are representative of the overall media set composition were selected consisting of 2400 frames of 1080p video drawn from 4 independent subjects, and 1200 frames of 4k video, also drawn from 4 independent subjects.  Restoration was restricted to the cropped face from detection. Any failure to detect a face thus reduces restoration and face processing time. Body detections occurred in 95\% of all frames, and faces were detected in 26\% of frames.

%\textcolor{red}{Can we combine this paragraph with the first paragraph of Sec. 4.1? }
%Experiments were conducted on a Dell Precision 5820, Intel Core i9-10980XE with 18 cores and 128 GB RAM, and 1 Nvidia RTX A6000.  During the test, GPU memory consumption remained consistently around 60\%, as did main memory consumption at just under 20\%. CPU usage was more variable but remained under 50\% during all observations.The experiments were repeated 30 times to generate the results. Excluding the first run where models are initialized, the variance of the total pipeline fps is 0.01.

%\textcolor{red}{examples of successful/unsuccessful verification and identification}


==> ref/sec_4_exp_v2.tex <==


\begin{table*}[t]
    \centering
\resizebox{0.90\linewidth}{!}{
    \begin{tabular}{|c||p{2.0cm}<{\centering}|p{1.8cm}<{\centering}||p{2.0cm}<{\centering}|p{1.8cm}<{\centering}||p{2.0cm}<{\centering}|p{1.8cm}<{\centering}|}
     \hline
      \multirow{2}{*}{Method} & \multicolumn{2}{c||}{ \makecell{\textbf{Verification (1:1)} \\ TAR@1\%FAR $\uparrow$} } & \multicolumn{2}{c||}{\makecell{\textbf{Rank Retrieval (1:N)} \\ Top20, Closed Search  $\uparrow$}}  & \multicolumn{2}{c|}{\makecell{\textbf{Open Search (1:N)} \\ FNIR@1\%FPIR $\downarrow$} } \\
      \cline{2-7}
      & FaceRestricted & FaceIncluded & FaceRestricted & FaceIncluded & FaceRestricted & FaceIncluded \\ 
      
     \hline\hline
 Baseline-AdaFace~\cite{kim2022adaface}     & 
 %24.95
 $9.61$ &  $66.20$ & $14.97$ & $73.85$ & $96.22$ & $70.64$ \\       
 \textbf{FarSight (Face)}    & 
 %25.04 
 $25.04$ & $78.01$ & $31.78$ & $84.12$ & $92.11$  & $57.39$\\     \hline  
 Baseline-GaitBase~\cite{gaitbase}    & $44.33$ & $45.55$ & $64.90$ & $68.03$ & $98.53$ & $98.79$ \\       
 \textbf{FarSight (Gait)}    & $56.23$ & $59.20$ & $72.55$ & $74.64$ & $95.24$ & $95.31$  \\   
 \hline  
 Baseline-CAL~\cite{CAL}         & $48.58$ & $51.87$ & $66.27$ & $71.18$ & $96.98$ & $96.17$\\       
 \textbf{FarSight (Body)}    & $51.02$ & $54.00$ & $69.18$ & $72.91$ & $96.95$ & $96.23$ \\     \hline
 \textbf{FarSight (Face+Gait)}     & $57.30$ & $83.98$  & $75.15$ & $91.19$ & $\textbf{87.64}$ & $\textbf{54.55}$ \\
\textbf{FarSight (Face+Body)}     & $54.68$ & $\textbf{85.93}$ & $73.97$ & $\textbf{93.13}$ & $89.57$ & $58.99$ \\ 
 \textbf{FarSight (Gait+Body)}     & $58.91$ & $62.08$ & $73.06$ & $75.57$ & $94.86$ & $94.74$\\ \hline \hline
  AdaFace+Gaitbase+CAL     & $61.05$ & $81.40$  & $75.20$ & $88.92$ & $90.80$ & $64.97$\\ 
   \textbf{FarSight}     & $\textbf{63.00}$ & $81.88$ & $\textbf{77.39}$  & $91.74$ & $90.66$ & $67.77$ \\  
 \hline
    \end{tabular}
    }
    \vspace{-2mm}
        \caption{Whole body biometric recognition results on the BRIAR dataset.}
	\label{tab:bts_results}
 \vspace{-2mm}
\end{table*}



\section{Experimental Results}\label{sec:exp} 

% BRIAR dataset paper https://openaccess.thecvf.com/content/WACV2023W/LRR/papers/Cornett_Expanding_Accurate_Person_Recognition_to_New_Altitudes_and_Ranges_The_WACVW_2023_paper.pdf

%{\color{red} All results should be obtained from our container using the BRIAR dataset (BGC1 + BGC2).}



%\subsection{Setting }
%  {\color{red} [ MSU]}

All modules are run together in a configurable container environment on PyTorch version 1.13.1. We perform experiments  on $8$ Nvidia RTX A6000s, with $48$ GiB of VRAM, over the course of $48$ hours on $2$ dual-socket servers with either AMD EPYC $7713$ $64$-Core or Intel Xeon Silver $4314$ $32$-Core processors.

\Paragraph{BRIAR Datasets and Protocols.}
%   {\color{red} [Feng, MSU]}
%
The BRIAR dataset~\cite{cornett2023expanding}, comprised of two collections—BRIAR Government Collections 1 (BGC1) and 2 (BGC2), is a pioneering initiative to support whole-body biometric research. It addresses the necessity for broader and richer data repositories for training and evaluating biometric systems in challenging applications. Using an array of imaging components, including DSLR cameras, surveillance systems, and UAV platforms, BRIAR consists of over $350,000$ images and $1,300$ hours of videos from $1,055$ subjects in outdoor settings.
%
The BRIAR dataset, with its focus on long-range and elevated angle recognition, provides a fertile ground for algorithm development and evaluation in whole-body biometrics.

The dataset has been partitioned into a training subset (BRS) and a testing subset (BTS) according to the provided Protocol V2.0.1. 
% 
For evaluation purposes, the probe sets have been categorized into two distinct groups: FaceIncluded and FaceRestricted. 
%
The FaceIncluded set comprises data where the face of the subjects is clearly visible, occupying a minimum of $20$ pixels in head height. %, with the width potentially varying due to changes in the yaw angle of the head. 
%
On the other hand, the FaceRestricted set consists of data that presents challenges such as occlusion, low resolution, or unusable faces. 
%%
These sets have been further subdivided into treatment and control sets to facilitate focused analysis. The control subset consists of cameras positioned at close range, typically within $75$ meters. 
%
These cameras are primarily used to establish performance expectations based on traditional methods. Conversely, the treatment sets comprise cameras situated at long distances or elevated angles, as well as UAVs. These configurations are of primary interest as they simulate real-world surveillance scenarios and pose greater challenges for biometrics. In conducting our experiments, we restrict the reported results to those from the treatment sets.



%%
\Paragraph{Metrics.}
\label{evaluation-metrics}
% {\color{green} [Minchul, MSU]}
We employ BRIAR Program Target Metrics~\cite{bba} to measure  FarSight's performance across multiple modalities and their fusion: 
%
verification (TAR@1\%FAR), closed-set identification (Rank-20 accuracy), and open-set identification (FNIR@1\%FPIR), allowing for a thorough examination of its performance across various settings. 
%
%Moreover, the system is evaluated in two modes -- face only and whole body.


%Verification is a task that assesses whether two given media, which can be images or videos, represent the same subject. In terms of performance metrics, one common measure is the Area Under the Curve (AUC) of match scores. AUC is a reliable indicator of the effectiveness of the verification system; a higher AUC (close to $1.0$) represents better separation between matches and non-matches. Additionally, to understand the performance at a specific operating point, True Acceptance Rate at a particular False Acceptance Rate (TAR@FAR) is often employed. In our discussions, we will use TAR@1\%FAR as an indicator of performance at a specific threshold.

%Identification is a task that involves recognizing an unknown individual (probe) from a known database (gallery). This task can be further divided into closed-set and open-set scenarios. In the closed-set scenario, all potential probe subjects are guaranteed to be present in the gallery. On the contrary, in the open-set scenario, the probe subjects may or may not be present in the gallery.

%For closed-set identification, the performance is usually measured by Rank-N accuracy. It is because closed-set search, alternatively known as Rank Retrieval, refers to an identification task where each probe has a corresponding match within the gallery of templates. In this scenario, given a probe video, the executing algorithm is tasked with returning the top R gallery matches that are associated with the probe.
%For instance, Rank-20 accuracy indicates how often the true match for a probe template is within the top 20 closest gallery templates. 

%The performance of a closed-set search can also be  quantified by the True Positive Identification Rate (TPIR) — representing the frequency at which the algorithm accurately retrieves a match for a probed template — and the False Negative Identification Rate (FNIR), which denotes the frequency of erroneous no-match returns by the algorithm for a probed template. A Cumulative Match Characteristic (CMC) curve, derived from these TPIR and FNIR values, succinctly encapsulates an identification algorithm's accuracy in matching search results and its proficiency in ranking the gallery results based on similarity.

%For open-set identification, performance is typically measured by the False Negative Identification Rate at a specific False Positive Identification Rate (FNIR@FPIR), specifically FNIR@1\%FPIR in our case.

%Through these metrics, we aim to assess the performance of our recognition pipeline across a variety of conditions and modalities including face, body, and gait. The corresponding performances will be summarized in the following sections.

\Paragraph{Baselines.}
%[{\color{green} Minchul \color{red} Ryan, Yiyang and Feng, MSU]}
%
In our study, we utilize established benchmarks for each biometric modality to ensure a comprehensive comparison: For facial recognition, we utilize AdaFace coupled with an average feature aggregation strategy, a popular approach known for its excellent performance~\cite{kim2022adaface}. For gait recognition, we adopt GaitBase~\cite{gaitbase}, a solution known for its efficacy. For body modality, we employ CAL~\cite{CAL}, a SoTA cloth-changing person re-identification method. These benchmarks provide an excellent basis to fairly evaluate our proposed method.

%In Tab.~\ref{tab:bts_results}, we provide the benchmark performance of publically available methods.  For the face modality, we use ArcFace~\cite{arcface} with the average feature aggregation as a benchmark. 
%For the gait modality, we use GaitBase~\cite{gaitbase} as our baseline. For the body modality, we use CAL~\cite{CAL}, SoTA Cloth-changing person re-identification method as our baselines.

\subsection{Evaluation and Analysis}

%{\color{red} Conducting Ablation Studies: Evaluating the Impact of Image Restoration and Detection on Biometric Recognition}

%We conduct an extensive comparison between our approaches and the baselines for each modality in Tab.~\ref{tab:bts_results}.
% 
%The detailed side-by-side analysis offers a clear perspective on our approaches' performance compared to the baselines.

In Tab.~\ref{tab:bts_results}, we provide a thorough comparison of our approaches and the baselines for each modality. The detailed comparison analysis clearly highlights the superior performance of our proposed FarSight system across all performance metrics when compared to the baselines.
%
For each modality, our module outperforms the baselines by a significant margin. For instance, in the verification metric (TAR@1\%FAR) on FaceIncluded sets, FarSight (Face) sees an increase of $11.81\%$. For gait, there's an improvement of $11.39\%$, and for body, we see an enhancement of $2.44\%$. Further, upon fusion, we gain an additional improvement of $6.77\%$ ($56.23\%\xrightarrow{}63.00\%$).

%
%We further investigate and report on the Rank-20 accuracy using the BRIAR dataset, taking into consideration differing altitudes and ranges. 
%
%As illustrated in Tab.~\ref{tab:bts_distance_results}, ....

\SubSubSection{Face}
% {\color{red} [Minchul, MSU]}
The efficacy of including various modules in the face recognition pipeline is shown in Tab.~\ref{tabl:faceparts}. We initially use the combination of AdaFace IR101 backbone with the average feature aggregation which has shown good performance in low-quality imageries~\cite{kim2022adaface}.  CFSM~\cite{liu2022cfsm} adds performance improvement by adopting training data to a low-quality image dataset WiderFace~\cite{widerface} ($+1.18$ in TAR@1\%FAR). CAFace~\cite{caface} is a feature fusion method which improves upon the basic average pooling (+$4.16$). Lastly, finetuning the model on the BGC1 training dataset further improves the performance (+$6.47$).  
%
The addition of image restoration using RTM based restoration model is shown in Tab.~\ref{tabl:facerestore}. The performance improvement is observed in the challenging \textit{FaceIncluded} group.
%However, for the easy \textit{face included control} group, the restoration is not helpful. 


\begin{table}[t]
    \centering
    \small
    \begin{tabular}{|c|c|c|c|}
    \hline
       FaceIncluded & \makecell{TAR@\\1\%FAR} & \makecell{Rank\\20} & \makecell{FNIR@\\1\%FPIR} \\ \hline
        AdaFace~\cite{kim2022adaface} & $66.20$ & $73.85$ & $70.64$ \\ \hline
         + CFSM~\cite{liu2022cfsm} & $67.38$ & $77.22$ & $68.51$ \\ \hline
         + CAFace~\cite{caface} & $71.54$ & $78.57$ & $61.77$ \\ \hline
        \makecell{+BRS1 \\FarSight (Face) }  &  $78.01$	& $84.12$	 & $57.39$   \\ \hline
        % \makecell{+Aligner} &  &  &  \\ \hline
    \end{tabular}
    \vspace{-2mm}
    \caption{Ablation of different parts in face recognition pipeline. }
    \label{tabl:faceparts}
    \vspace{-2mm}
\end{table}



\begin{table}[t!]
    \centering
    \small
    \begin{tabular}{|r|c|}
    \hline
       TAR@1\%FAR  & \makecell{FaceIncluded} \\ \hline
        Face w/o Restoration  & $72.39$\\ \hline
        Face w/ Restoration   &$\mathbf{72.57}$ \\ \hline
        % \makecell{+Aligner} &  &  &  \\ \hline
    \end{tabular}
    \vspace{-2mm}
    \caption{Face recognition with and without image restoration.}
    \label{tabl:facerestore}
    \vspace{-2mm}
\end{table}

%-------------------------------------------------------%
\SubSubSection{Gait}
% {\color{red} [Ryan and Yiyang, MSU]}
% \paragraph{FarSight-Gait vs. GaitBase~\cite{gaitbase}.}
In our gait recognition experiments, we observe consistent improvements compared to GaitBase~\cite{gaitbase}, our baseline, across all four metrics.
%
Our findings demonstrate significant enhancements in the model's ability to accurately verify individuals, with the TAR@1\%FAR reaching an impressive improvement of \(11.90\%\) in FaceRestricted verification and \(13.65\%\) in FaceIncludd verification. 
%
Further, the top-20 rank metric exhibits notable advancement, showcasing a remarkable increase of \(6.61\%\) compared to our baseline. 
%
Lastly, our model showcases improved performance in open-set search, achieving a noteworthy reduction of \(3.29\%\) in FNIR@1\%FPIR.
%
These promising outcomes reaffirm the efficacy of FarSight (Gait) to extract more discriminative features based on global features and highlight its potential for reliable and robust biometric identification in real-world applications.

%-------------------------------------------------------%
\SubSubSection{Body}
Table~\ref{tab:bts_results} clearly demonstrates that our FarSight (body) consistently outperforms the CAL baseline on both FaceRestricted and FaceIncluded sets, as evidenced in both verification and Rank retrieval metrics.

% {\color{red} [Feng, MSU]}
%\noindent\emph{Body matching vs. Gait recognition.} The performance of body matching and gait recognition varies depending on conditions. As shown in Tab.~\ref{tab:bm_mission_results_comparison}, gait recognition outperforms body in turbulent, low-resolution situations, thanks to its resilience. On the other hand, body matching excels in elevated views, where the 3D body shape can still be deduced even when gait becomes less distinguishable.

\noindent\emph{Body Matching Observations.}
In Fig.~\ref{fig:body_matching_paired_examples}, we show succeeded and failed matches in body matching. Our method copes well with clothing differences, but struggles with motion blur, turbulence, or hairstyle changes. Misidentifications in impostor pairs often happen due to similar body shapes.

%\begin{table}[t!]
%\small
%\centering
%\resizebox{0.98\linewidth}{!}{
%\begin{tabular}{|l|c|c|c|c|c|}
%\hline 
%Mission     &Metric      & \textbf{FarSight (Gait)}   & \textbf{FarSight (Body)}  \\
%\hline 
%LR Turbulence   & \multirow{2}{*}{Rank20 $\uparrow$}  &  $\textbf{74.77}$ & $75.54$ \\
%Elevated        &   &  $75.25$ & $\textbf{72.18}$ \\
%\hline 
%    LR Turbulence   &  \multirow{2}{*}{TAR@1\%FAR $\uparrow$} & $\textbf{59.69}$ & $56.53$ \\
%Elevated        &   & $57.68$ & $\textbf{52.82}$      \\
%\hline\hline
%LR Turbulence   &  \multirow{2}{*}{ FNIR@1\%FPIR} & $98.41$   & %$\textbf{97.95}$ \\
%Elevated        & & $96.97$   & $\textbf{96.05}$    \\
%\hline
%\end{tabular}
%}
%\vspace{-2mm}
%\caption{\small Comparison between body matching and gait recognition on Mission LR Turbulence and Elevated: the two missions where neither modality has the most advantage.}
%\label{tab:bm_mission_results_comparison}
%\vspace{-2mm}
%\end{table}

\begin{figure}[t!]
\begin{center}
\resizebox{1\linewidth}{!}{
\begin{tabular}{c c c c c}
{\includegraphics[height=3cm]
{fig/Feng/pairs/hs_genuine/BTS1.0_G00003_field_0000114712____BTS1_G00003_controlled_0000002844____1.0601.png}} & 
{\includegraphics[height=3cm]{fig/Feng/pairs/hs_genuine/BTS1.0_G00071_field_0000118399____BTS1_G00071_controlled_0000002938____1.143.png}} &
{\includegraphics[height=3cm]{fig/Feng/pairs/hs_genuine/BTS1.0_G00073_field_0000119810____BTS1_G00073_controlled_0000001413____1.1114.png}} &
{\includegraphics[height=3cm]{fig/Feng/pairs/hs_genuine/BTS1.0_G00293_field_0000136963____BTS1_G00293_controlled_0000004716____1.0602.png}} &
{\includegraphics[height=3cm]{fig/Feng/pairs/hs_genuine/BTS1.0_G00448_field_0000157658____BTS1_G00448_controlled_0000005519____1.1014.png}}  \\
\multicolumn{5}{c}{\LARGE (a) Successful Recognition of Genuine Pairs}\vspace{3mm}\\ 
{\includegraphics[height=3cm]{fig/Feng/pairs/ls_impostor/BTS1.0_G00083_field_0000121633____BTS2_G02678_controlled_0000041763____-0.60766.png}} & 
{\includegraphics[height=3cm]{fig/Feng/pairs/ls_impostor/BTS1.0_G00246_field_0000130545____BTS2_G02529_controlled_0000032686____-0.64466.png}} &
{\includegraphics[height=3cm]{fig/Feng/pairs/ls_impostor/BTS1.0_G00380_field_0000150022____BTS2_G02682_controlled_0000042160____-0.61029.png}} &
{\includegraphics[height=3cm]{fig/Feng/pairs/ls_impostor/BTS2.0_G02005_field_0000551568____BTS1_G00143_controlled_0000005168____-0.61122.png}} &
{\includegraphics[height=3cm]{fig/Feng/pairs/ls_impostor/BTS2.0_G02053_field_0000578230____BTS1_G00236_controlled_0000007772____-0.60312.png}}  \\
\multicolumn{5}{c}{\LARGE (b) Successful Recognition of Impostor Pairs}\vspace{3mm}\\
{\includegraphics[height=3cm]{fig/Feng/pairs/ls_genuine/BTS1.0_G00026_field_0000116303____BTS1_G00026_controlled_0000003233____-0.038741.png}} & 
{\includegraphics[height=3cm]{fig/Feng/pairs/ls_genuine/BTS1.0_G00162_field_0000123789____BTS1_G00162_controlled_0000012232____0.17941.png}} &
{\includegraphics[height=3cm]{fig/Feng/pairs/ls_genuine/BTS2.0_G02011_field_0000552533____BTS2_G02011_controlled_0000013408____0.20464.png}} &
{\includegraphics[height=3cm]{fig/Feng/pairs/ls_genuine/BTS2.0_G02052_field_0000575654____BTS2_G02052_controlled_0000007329____0.16695.png}} &
{\includegraphics[height=3cm]{fig/Feng/pairs/ls_genuine/BTS2.0_G02063_field_0000582889____BTS2_G02063_controlled_0000000524____0.17496.png}}  \\
\multicolumn{5}{c}{\LARGE (c) Failure Cases for Genuine Pairs}\vspace{3mm}\\
{\includegraphics[height=3cm]{fig/Feng/pairs/hs_impostor/BTS1.0_G00003_field_0000114924____BTS1_G00044_controlled_0000001130____1.0442.png}} & 
{\includegraphics[height=3cm]{fig/Feng/pairs/hs_impostor/BTS1.0_G00134_field_0000122985____BTS1_G00071_controlled_0000002938____1.0872.png}} &
{\includegraphics[height=3cm]{fig/Feng/pairs/hs_impostor/BTS1.0_G00286_field_0000136103____BTS1_G00124_controlled_0000004193____1.0882.png}} &
{\includegraphics[height=3cm]{fig/Feng/pairs/hs_impostor/BTS1.0_G00469_field_0000160417____BTS1_G00393_controlled_0000017635____1.0609.png}} &
{\includegraphics[height=3cm]{fig/Feng/pairs/hs_impostor/BTS1.0_G00550_field_0000169999____BTS1_G00304_controlled_0000008032____1.0825.png}}  \\
\multicolumn{5}{c}{\LARGE (d) Failure Cases for Impostor Pairs}\\
\end{tabular}
}
\end{center}
\vspace{-5mm}
\caption{\small Examples of successful recognition and failure cases of genuine and impostor pairs in body matching.
} 
\label{fig:body_matching_paired_examples}
\vspace{-2mm}
\end{figure}

%-------------------------------------------------------%
%\subsubsection{Multi-Modality Fusion}
\SubSubSection{Multi-Modal Fusion}

As seen in Tab.~\ref{tab:bts_results}, fusion of the three modalities provides a significant increase over the next best performing single modality, particularly in the face restricted conditions ($+18.18$ in TAR@1\%FAR and $+13.25$ in Top20). We see also that dual-modality results are outperformed by FarSight in all but one metric (FNIR@1\%FPIR), highlighting the benefit of our proposed three-modality system.
% {\color{red} [Ryan, MSU]}

\SubSubSection{System Efficiency}
%{\color{red} [Chris, MSU]}
 
%Feature vectors for face, gait and body are of sizes 512, 7936 and 6144. Multiplying these values by 8 and dividing by 128 provides us with the template sizes: $4$KB, $62$KB and $48$KB, respectively. and $114KB
%\begin{table}
%    \centering
%    \begin{tabular}{|c|c|c||c|}\hline
%                      Body & Face & Gait & Combined \\\hline
%       $48$ & $4$ & $62$ & $114$\\\hline
%    \end{tabular}
%    \caption[Template sizes.]{Template sizes (KB).}
%    \label{tab:size}
%\end{table}
%
\Paragraph{Template sizes.} Feature vectors for face, gait and body are of sizes $512$, $7936$ and $6144$. Multiplying these values by $8$ and dividing by $128$ provides the template sizes: $4$KB, $62$KB and $48$KB, respectively, and $114$KB in total.
%

\Paragraph{Processing speed.} The speed of our FarSight system, as outlined in Tab.~\ref{tab:processing_time}, is examined under stringent conditions to gauge both the efficiency of individual components and the overall pipeline. 
This system operates asynchronously and concurrently, similar to the actual deployment conditions. 
To precisely measure efficiency, the components are assessed in a serialized manner, even though they typically run in parallel.
%
We conduct this assessment using representative sample videos, encompassing $2400$ frames of $1080$p and $1200$ frames of $4$K video, each set originating from four distinct subjects. 
The restoration process is primarily directed towards detected faces, which implies that any instances of undetected faces would naturally lead to reduced restoration and face module processing times. A notable observation is that our system can successfully detect bodies in $95$\% of all frames and faces in $26$\% of frames.

%Processing speed statistics are displayed in Tables~\ref{tab:processing_time} and ~\ref{tab:speed_pipeline}. Module components run asynchronously and concurrently in the deployed pipeline. To isolate component efficiency, an evaluation is executed by processing pipeline components serially rather than concurrently.  Individual component efficiency is displayed in seconds and overall pipeline performance is represented in frames per second (fps).


\begin{table}
    \centering
    \resizebox{0.9\linewidth}{!}{
    \begin{tabular}{|c|c|c|c|}\hline
        Module & 1080p & 4K & Average Combined\\ \hline \hline
        Detection \& Tracking & $20.0$ & $34.7$ & $24.9$ \\ \hline
        Restoration           & $6.1$  & $5.3$  & $5.9$\\ \hline
        Face                  & $2.6$  & $2.2$  & $2.5$\\ \hline
        Gait                  & $3.3$  & $2.5$  & $3.0$\\ \hline
        Body                  & $3.7$  & $3.1$  & $3.5$\\ \hline \hline
        FarSight system & $8.4$ & $6.3$ &  $7.8$\\ \hline
    \end{tabular}
    }
    \vspace{-2mm}
    \caption{\small Efficiency (fps) of each FarSight system module.}
    \label{tab:processing_time}
    \vspace{-4mm}
\end{table}

%\begin{table}
%    \centering
%    \begin{tabular}{|c|c|c|c|}\hline
%        Media              & 1080p & 4K & Average Combined \\ \hline
%        Speed (fps) & $8.4$ & $6.3$ &  $7.8$\\ \hline
%    \end{tabular}
%    \caption{Average Speed of Frame Processing in our FarSight.}
%    \label{tab:speed_pipeline}
%\end{table}

%Sample videos that are representative of the overall media set composition were selected consisting of 2400 frames of 1080p video drawn from 4 independent subjects, and 1200 frames of 4k video, also drawn from 4 independent subjects.  Restoration was restricted to the cropped face from detection. Any failure to detect a face thus reduces restoration and face processing time. Body detections occurred in 95\% of all frames, and faces were detected in 26\% of frames.

%\textcolor{red}{Can we combine this paragraph with the first paragraph of Sec. 4.1? }
%Experiments were conducted on a Dell Precision 5820, Intel Core i9-10980XE with 18 cores and 128 GB RAM, and 1 Nvidia RTX A6000.  During the test, GPU memory consumption remained consistently around 60\%, as did main memory consumption at just under 20\%. CPU usage was more variable but remained under 50\% during all observations.The experiments were repeated 30 times to generate the results. Excluding the first run where models are initialized, the variance of the total pipeline fps is 0.01.

%\textcolor{red}{examples of successful/unsuccessful verification and identification}


==> ref/sec_5_conclusion_v1.tex <==

\section{Future Research}
% {\color{red} [Purdue, UT Austin, UO and MSU]}

\begin{itemize}[leftmargin=*]
\item  Image restoration. Three directions of image restoration are currently being pursued. Firstly, we are expanding the capability of the optical simulation tool to handle distortions beyond atmospheric turbulence. These include color aberration, motion blur, out-of-focus, and lost contrast due to haze and fog. Secondly, we are exploring the possibility of ``simulation-in-the-loop'' where the reconstruction algorithm can seamlessly use the simulation too within the inverse formulation. Thirdly, we are exploring how to jointly perform restoration-recognition co-optimization. In addition, we are also exploring to combine the benefits of generative image restoration techniques (eg, diffusion based) with conventional discriminative approaches to simultaneously improve the fidelity and perceptual quality of the restoration.
%
\vspace{-3mm}\item  Detection and tracking. Detection and tracking is currently imposing a noticeable bottleneck on the entire pipeline, which we aim to avoid in the future by either optimizing the region-based detector, or switching to YOLO-based detectors entirely. However, this would require careful evaluation of the entire pipeline, as well as detection performance itself. In addition, when considering detectors where joint body and face detection is not directly applicable, additional post-processing will be required to associate face and body detections. Depending on the latency of the detector, another possible avenue is to detect subjects first, and then use a separate face detector on the extracted bounding box from the subject, which would bear lower latency from the lower resolution, to detect face bounding boxes.
%
\vspace{-3mm}\item  Biometric feature encoding. For face module, the analysis on the effect of restoration tells us that blindly improving the image quality can negatively impact the performace. In future works, we can look into adaptive restoration that restores images when it has enough information from the given frames. For the body module, we plan to refine the accuracy of 3D nude body reconstruction by using multiple frames in the body matching framework. This method, which takes advantage of multiple observations, enhances body matching precision by effectively handling variations in pose, lighting, and occlusion. Thus, the improved discriminative 3D identity features contribute significantly to body matching.
% gait recognition
Besides, as we have seen that 3D body modeling is beneficial for body matching, it becomes a natural question whether the 3D poses can also provide complementary information to 2D skeletons or imageries.
\vspace{-3mm}\item  Multi-modality fusion.
\end{itemize}



\section{Conclusion}\label{sec:conclusion}
% {\color{red} [Feng, MSU]}

In this work, we develop a new system, \textbf{FarSight}, which stands as a beacon of progress in whole-body biometric recognition. The solution ingeniously overcomes hurdles such as low-quality video frames, large yaw and pitch angles, and the disparity between training and test sets by utilizing the physics of imaging in harmony with deep learning models. This innovative approach has led to superior recognition performance, as demonstrated in tests using the BRIAR dataset. With the far-reaching potential to enhance security surveillance and forensic identification, the FarSight system paves the way for the next generation of biometric recognition.

==> sec_3_method_submission.tex <==


\Section{FarSight: System Architecture}\label{sec:}

\SubSection{Overview of FarSight}
% {\color{red} [Chris, MSU]}
%%
As illustrated in Fig.~\ref{fig:overview}, FarSight operates through six modules: detection and tracking, image restoration, face, gait, and body shape feature extraction, and multi-modal fusion. These modules work within a scalable testing framework, optimizing GPU usage via adaptable batch sizes.
%
An API utility facilitates communication between the framework and external systems, transmitting video sequences from configuration files to the framework via Google RPC calls. Essential features extracted from these sequences are stored in HDF5 files for performance evaluation.

The workflow starts with the detection and tracking modules processing the input video sequences. Bounding boxes indicating regions of interest (RoI) are cropped and sent to the gait and body modules, while the face images are restored before processing. The body and gait modules generate unique per-sequence feature vectors through average pooling, while the face module uses CAFace~\cite{caface} to consolidate features across video sequences.
%
A probe is composed of single video segments per subject. On the other hand, gallery enrollments - consisting of multiple video sequences and still images - are processed and combined into a singular subject-level feature vector for each modality.

%As shown in Fig.~\ref{fig:overview}, the FarSight system operates through an intricate assembly of six modules, each tailored for a specific function: detection and tracking, image restoration, three biometric modalities, namely, face, gait, and body feature extraction, and multi-modality fusion module. These modules function within a containerized testing framework, utilizing GPU resources effectively through dynamically adjustable batch sizes.

%%
%An API utility bridges the interaction between the framework and external systems, streaming video sequences identified from configuration files to the testing framework using Google RPC calls. The framework then extracts vital features from these sequences, which are stored in HDF5 databases for match performance evaluation.

%%
%The workflow begins with video sequence processing through the detection and tracking modules. Bounding box-detected images are cropped and dispatched to the gait and body feature encoding module. Simultaneously, the cropped face frames undergo image restoration before their delivery to the face module. 
%
%Both the body and gait modules produce a unique per-sequence feature vector from a single run of all sequences via average pooling operation, while the face pipeline employs CAFace~\cite{caface} to aggregate the features across various sequences.

%%
%Catering to the varying needs of enrollments, the system processes probe enrollments as single video segments per subject, generating definitive feature vectors. Conversely, gallery enrollments, composed of multiple video sequences and still images, undergo additional consolidation, merging into a singular, comprehensive subject-level feature vector post-processing.

%\noindent 
%The FarSight system is comprised of five modules that provide functions for detection and tracking, image restoration, and the three biometric modalities: body extraction, face extraction and gait extraction.  Each module is wrapped in a standard interface and deployed in containerized testing framework.

%The testing framework listens for calls to standard functions for gallery and probe enrollment into a database, database manipulation functions for merging and finalizing, and scoring functions to generate raw matching data that can subsequently be processed to generate performance results.

%Calls to the testing framework originate via an API utility that takes configuration files that identify gallery and probe source media and streams media to the testing framework over Google RPC calls in a frame-by-frame manner.  Still images (gallery only) and videos (both gallery and probe) are submitted to the test framework for feature extraction and the framework writes extracted features out to databases in the HDF5 format. These databases can then be utilized to determine matching performance.

%Each module is executed asynchronously in its own process space, allowing for different batch sizes for each module to make best use of available GPU resources.  Results are synchronized at the end of processing of each media piece.

%Media is first sent to the detection and tracking modules and fed to subsequent modules, following appropriate pre-processing, as detection and tracking results become available.  Frame-by-frame image data and corresponding detection bounds are first pre-processed into appropriately cropped and scaled batches before sending to the body and gait modules.  Image restoration is applied to face frames before sending to the face module.  Both restored and unrestored imagery is sent to the face module to allow it to make a best-result judgement on which form to use.

%Body and gait both process all images in each discrete media in a single pass resulting in a single per-media feature vector respectively.  In contrast, the face pipeline processes in two stages, first generating intermediate AdaFace feature vectors for each frame in the source media, and then passing those intermediate feature vectors to CAFace to generate a resulting feature vector.

%Probe enrollments consist of a single video segment per subject, and thus the resulting feature vectors above are final.  Gallery enrollments, however, consist of multiple video and still images and the media-level feature vectors must be finalized into a single subject-level feature vector once all gallery media has been processed.
%Fig.~\ref{fig:overview} 




\SubSection{Challenges in FarSight}
%{\color{red} [Feng, MSU]}

%Our FarSight system faces an array of unique challenges.
%
%Firstly, long-range capture and atmospheric turbulence often result in low-quality biometric samples that are difficult to process. Secondly, elevated platforms introduce large yaw and pitch angles, further complicating the data analysis. Additionally, the low visual quality hampers the extraction of identity information, making accurate recognition more difficult. The training data also presents a limitation, as its domain is restricted due to diverse environmental changes. Lastly, the low generalizability and explainability of deep learning models pose a significant challenge to the achievement of reliable and transparent results. 
%
%In Fig.~\ref{fig:briar_examples}, we provide examples from close-range, mid-range (100m-500m), and UAV scenarios for a more visual understanding of these challenges. 

The FarSight system faces distinct challenges. 
Captured videos often suffer from poor quality due to long-range capture and atmospheric turbulence.
Elevated platforms introduce large yaw and pitch angles, making data analysis more challenging. 
Extracting identity features is affected by low visual quality, and the training data's limited domain further complicates the learning task. 
Further, the lack of transparency in deep learning models poses a significant issue. Fig.~\ref{fig:briar_examples} illustrates these challenges with examples from close-range, mid-range ($100$-$500$m), and UAV-captured scenarios.

\SubSection{Physics Modeling of Turbulence}

\noindent Atmospheric turbulence is an unavoidable degradation when imaging at range. It is often computationally modeled by splitting the continuous propagation paths into segments via phase screens as illustrated in Fig.~\ref{fig: turbulence simulation}. 
While accurate, the spatially varying nature of the propagation
%For \emph{every} point on the object plane, we need to perform a series of Fourier transforms and phase multiplications to compute the point spread function on the image plane \cite{Hardie_2017_a, Hardie_2022_a, Schmidt_2010_a}. 
makes this a computationally demanding process \cite{hardie2017simulation, Hardie_2022_a, Schmidt_2010_a}.

\begin{figure}[t]
\begin{center}
\includegraphics[trim={0 0 0 7.2cm},clip, width=0.95\linewidth]{fig/Feng/fig3_briar_examples.pdf}
\end{center}
\vspace{-6mm}
   \caption{\small Example frames in the BRIAR dataset~\cite{cornett2023expanding} showing the same subject (identity) under various conditions, including different standoff distances, clothing, and image quality due to the turbulence effect. The columns represent different scenarios: controlled conditions, close range, $100$m-set1, $100$m-set2, $200$m, $400$m, $500$m, and UAV capture, respectively.}
\label{fig:briar_examples}
\vspace{-5mm}
\end{figure}
%The four subjects shown here (one per row) in the figure (ID: G02030, G02062, G02217 and G02229) consented to have their images included for publication.




More recent works have explored the possibility of \emph{propagation-free} models where the turbulence effects are implemented as random sampling at the \emph{aperture} \cite{Chimitt_2020_a, Mao_2021_a, chimitt_2022_a}. As shown in Fig.~\ref{fig: turbulence simulation}, every pixel on the aperture is associated with a random phase function which has a linear representation using the Zernike polynomials \cite{Noll_1976_a}. By constructing the covariance matrix of the random process, we can draw samples of the Zernike coefficients to enforce spatial and modal correlations. Propagation-free simulation has enabled $1000 \times $ speed up compared to the split-step propagation methods while maintaining accuracy. Therefore, we adopt this simulation approach in our system.
%This will lead to two principal components of the turbulent effects: (1) tilt (i.e., geometric displacement of pixels) and (2) spatially varying blur \cite{Chan_2022_a},
% \begin{equation}
%     I(\mathbf{x}) = [\mathcal{B} \circ \mathcal{T}] (J(\mathbf{x})),
%     \label{eq: turb_img_form}
% \end{equation}
% where $\mathcal{T}$ is the tilt operator and $\mathcal{B}$ represents the blur operation, with $J(\mathbf{x})$ and $I(\mathbf{x})$ as the input and output images, indexed by position $\mathbf{x}$, respectively. 




For the generation of training data, realistic optical and turbulence parameters significantly influence the appearance of the generated defects. Therefore, our datasets are synthesized according to the metadata of various long-range optical systems. Our training dataset also consists of both dynamic and static scenes \cite{Safdarnejad_2015_a, Jin_2021_a, zhou2017places}. 


 %Solving the inverse problem of \eqref{eq: turb_img_form} is highly non-trivial and deviates from many classical deblurring problems \textcolor{red}{[a few citations]}, where blur is assumed to be uniform or the shifting to be global. 


% For learning-based restoration, imaging through turbulence poses a significant problem: ground truth is almost \emph{never} available -- if the image is observed through turbulence at one instance, we cannot ``turn it off'' in the next. Therefore, reliance on simulation for restoration is essential. Although existing methodologies exist \textcolor{red}{[split-step works]}, generating a sufficient amount of data is likely infeasible as noted by Chimitt et al. .
% %the generation a 4k dataset consisting of 1000 sequences with 100 frames each will take 156 years to process using split-step based methods.



%The series of works describing Zernike-based simulation  succeed in maintaining accuracy while increasing the speed by a factor of $\times\!1000$. Although the capability exists, proper selection of parameters and application to images in training is non-trivial. Improper application will overemphasize certain aspects such as pixel shifting or blur size, therefore, to accurately represent imaging through turbulence, we must choose the parameters carefully. Because we are specifically interested in biometric recognition, we can tailor our parameter choices for simulation to reasonably match our expectation for where our restoration may be applied. Exact parameter choices can be found in the supplementary document. The types of scenes we focus are fairly general, simulating on a few video datasets \cite{Safdarnejad_2015_a, Jin_2021_a, zhou2017places}.






\SubSection{Detection and Tracking}
% {\color{green} [UO team]}
%%%% Will redo equations to avoid overflowing
%%%% Figures will be added soon.


Our detection module, based on~\cite{wan2021bodyface}, uses a two-stage R-CNN detector~\cite{ren2015faster} with a modified ResNet50 backbone to associate face and body bounding boxes~\cite{wan2021bodyface}. This is done using associative embeddings to match faces and bodies, learned via \textbf{pulling} and \textbf{pushing} loss functions~\cite{duan2019centernet}.
%
The pulling loss brings embeddings of the same subject closer in the presence of intra-subject variations, calculated as body-to-body, face-to-face, and face-to-body pairs. These are combined using a weighted sum of body-to-face loss, and the sum of face-to-face and body-to-body losses.
%
Pushing loss, in contrast, pushes away bounding boxes assigned to different subjects to account for inter-subject variations. It is divided into three losses between pairs of body boxes, pairs of face boxes, and body-face pairs. These losses are combined by a weighted sum.
%
The final associative embedding loss used to optimize these embeddings is a weighted sum of the pulling and pushing losses.

The module also predicts ``head hook" coordinates for every subject to improve body and face association. The head hook loss is a weighted sum of the Smooth L1 loss~\cite{girshick2015fast} and a scale-invariant angular loss.
%
The final association between body and face bounding boxes is based on similarity metrics, including embedding distance, head hook distance, and confidence scores. The RBF kernel is used for both the embedding distance and head hook distance. The confidence scores factor directly into the association loss to mitigate associating low-confidence bounding boxes with high-confidence ones.
%
Finally, all these metrics are integrated into a final association metric. If a face prediction's maximum similarity score with any body is below a set threshold, it is concluded that the subject's face is not visible.



\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{./fig/turbulence/turb_simulation.pdf}
\vspace{-4mm}
\caption{\small Turbulence modeling. Comparing split-step~\cite{hardie2017simulation,bos2012technique} and Zernike-based simulations \cite{Chimitt_2020_a, Mao_2021_a, chimitt_2022_a}.}
\label{fig: turbulence simulation}
\vspace{-3mm}
\end{figure}






\SubSection{Image Restoration} 

Image restoration aims to reverse the image formation process, as described by the equation~\cite{Chan_2022_a}
\begin{equation}
    I(\mathbf{x}) = [\mathcal{B} \circ \mathcal{T}] (J(\mathbf{x})),
    \label{eq: turb_img_form}
\end{equation}
where, $\mathcal{T}$ is the tilt operator and $\mathcal{B}$ represents the blur operation, with $J(\mathbf{x})$ and $I(\mathbf{x})$ as the input and output images, indexed by position $\mathbf{x}$, respectively. In this work, we have considered a single-frame image restoration method as well as a multi-frame method, both aiming to invert $\mathcal{T}$ and $\mathcal{B}$. 


Our restoration methods for biometrics focus on preserving identity, using lightweight, real-time techniques. These are divided into single-frame and multi-frame restorations. The former provides lower throughput but relies on strong priors without altering the subject's identity. Multi-frame restoration, on the other hand, utilizes temporal cues, allowing weaker priors but requiring larger throughput.


Our multi-frame approach uses the Recurrent Turbulence Mitigation network (RTM), a bi-directional, multi-scale convolutional recurrent network with a novel Multi-head Temporal Channel self-attention (MTCSA) layer (Fig.~\ref{fig: rtm}).
%
%For single-frame restoration, we employ Turbulence Mitigation Network (TurbNet~\cite{Mao_2022_a}), which estimates turbulence distortion during restoration (Fig. \ref{fig: TurbNet}). After restoration, the estimate is re-distorted for prediction evaluation.


\begin{figure}[t]
    \centering
    \includegraphics[width = 0.9\linewidth]{fig/turbulence/RTM_figure.pdf}
    \vspace{-2mm}
    \caption{\small Multi-frame image restoration by the recurrent network for turbulence mitigation (RTM).}
    \label{fig: rtm}
\vspace{-2ex}
\end{figure}


%\begin{figure}[t]
%    \centering
%    \includegraphics[width = \linewidth]{fig/turbulence/main_arch_eccv}
%    \vspace{-6mm}
%    \caption{\small Single-frame image restoration by TurbNet.}
%    \label{fig: TurbNet}
%\vspace{-3ex}
%\end{figure}












\SubSection{Multi-Modal Biometric Feature Encoding} %{\color{red} [Ryan and Feng, MSU]}}

We describe here our methods for obtaining biometric features from the face, gait and body shape, as well as the multi-modal fusion technique applied to generate fused scores for evaluation on the metrics described in Sec.~\ref{evaluation-metrics}.
\SubSubSection{Face}
\label{face-feature-encoding}
%{\color{green} [Minchul, MSU]}
Our face recognition pipeline integrates the techniques of Adaptive Margin Function (AdaFace~\cite{kim2022adaface}), Cluster and Aggregate (CAFace~\cite{caface}), and Controllable Face Synthesis Model (CFSM~\cite{liu2022cfsm}), addressing the challenge of recognizing faces across variable image qualities and media types.

Initially, AdaFace~\cite{kim2022adaface}, an adaptive loss function strategy, helps manage low-quality face datasets. It adjusts the emphasis on misclassified samples based on image quality, effectively dealing with a wide range of image quality levels.
%
Next, CAFace~\cite{caface}, a two-stage feature fusion technique, is crucial for integrating features from multiple frames. By grouping inputs to a few global cluster centers and subsequently fusing these features, CAFace maintains order invariance while combining multiple frames.
%
Lastly, CFSM~\cite{liu2022cfsm} helps bridge domain gaps between training and testing scenarios. It replicates the target datasets' distribution in a style latent space, generating synthetic face images similar to the target evaluation datasets, thereby reconciling the disparity between high-quality training data and lower-quality surveillance images.
%
The combination of AdaFace, CAFace, and CFSM effectively navigates the challenges of face recognition across diverse image qualities, leveraging feature extraction, feature integration, and synthetic image generation to improve face recognition performance.

%Herein, we describe our face recognition pipeline that incorporates the methods of AdaFace~\cite{kim2022adaface}, CAFace~\cite{caface}, and CFSM~\cite{liu2022cfsm}, creating a comprehensive approach to overcome the challenges of recognizing faces across varied image qualities with both image and video media.

%Our pipeline initiates with AdaFace~\cite{kim2022adaface}, an adaptive loss function technique designed for handling low-quality face datasets. The framework uses image quality to adaptively modulate the emphasis on misclassified samples, a feature particularly effective for managing the wide range of image qualities.

%Further enhancement of our pipeline involves the implementation of CAFace~\cite{caface}, a two-stage feature fusion paradigm that is indispensable for incorporating features across multiple frames. By assigning inputs to a limited number of global cluster centers and later fusing the clustered features, CAFace provides the ability to combine multiple frames while maintaining order invariance.

%Lastly, our pipeline incorporates the Controllable Face Synthesis Model (CFSM)~\cite{liu2022cfsm}. Given the persistent challenge of domain gaps between semi-constrained training datasets and unconstrained testing scenarios, CFSM provides a solution by mimicking the target datasets' distribution in a style latent space. This face synthesis model allows for precise control over the diversity and degree of synthesis, and the pre-trained synthesis model is designed to be guided by the FR model, generating images that are more beneficial for FR model training. Crucially, this approach allows us to generate synthetic face images similar in style to the target evaluation datasets, bridging the gap between high-quality training data and lower-quality surveillance images.

%The amalgamation of AdaFace, CAFace, and CFSM within our pipeline forms a comprehensive solution to the challenges of face recognition across a diverse range of image qualities. Through effective frame-level feature extraction, integration of these features, and controllable synthetic image generation, our approach achieves substantial improvements in face recognition tasks across both high and low-quality image datasets.

\SubSubSection{Gait}
%{\color{red} [Yiyang, MSU]}

We propose an innovative framework, GlobalGait, to address the limitations of existing gait recognition models that mainly focus on local features and often overlook vital global correlations. GlobalGait enriches these local features by factoring in global correlations across a gait sequence, thereby boosting recognition accuracy.

Given an input sequence, GlobalGait uses a CNN backbone to extract local spatiotemporal features, and then divides them into source and target features. These feature maps are projected into tokens for each joint, using sampling around each 2D joint. We employ a stack of multi-head self-attention layers to model the sequences' spatial and temporal correlations.
%
Further, GlobalGait attempts to reconstruct target frame pixels based on source sequences and to choose the correct target sequence from a set of candidates. 
This approach harnesses the spatial and temporal correlations in gait recognition, with these supervisory signals guiding the model to learn more distinct gait features.

%Gait recognition is a biometric technique that focuses on analyzing an individual's walking patterns and movements to identify and differentiate them from others. 
% Unlike other biometric modalities like facial recognition, gait patterns can be captured from a distance and/or altitude.
%It is particularly advantageous for long-distance and high-altitude surveillance applications, such as surveillance cameras mounted on buildings and unmanned aerial vehicles (UAVs), due to its ability to capture and analyze gait patterns from a distance. 
%Unlike other biometric modalities like facial recognition, gait recognition can work effectively even when the subject's face is obscured, making it valuable in long-range and aerial scenarios. 
%Additionally, gait recognition takes advantage of the dynamic nature of walking, capturing the unique rhythm, pace, and motion characteristics exhibited by individuals while other biometric modalities such as face recognition and body matching primarily rely on static features.
%Focusing on the inherent temporal cues of gait enhances the accuracy and reliability of biometric identification in scenarios where other modalities may fall short.

%Through our observations, we have identified a limitation in the current state-of-the-art gait recognition models, specifically their predominant focus on extracting local gait features while neglecting the essential global correlations. These global correlations refer to the interdependencies between different body parts across various frames of a gait sequence. In order to address this limitation and enhance the discriminability of gait recognition, we propose an innovative framework named GlobalGait. This framework aims to enrich the local gait features by incorporating and leveraging the crucial global correlations, thereby improving the overall effectiveness and accuracy of gait recognition.

%In particular, given an input sequence \(\left(\mathbf{I}_1, \mathbf{I}_2, \dots, \mathbf{I}_{N}\right)\), we first use a CNN backbone to extract local spatiotemporal features \(\mathbf{F}_{\mathit{backbone}}\), which is then divided into \(\mathbf{F}_{\mathit{source}}\) and \(\mathbf{F}_{\mathit{target}}\). 
%We project the feature maps to tokens \(\mathbf{T}\) for each joint by sampling around each 2D joint. 
%And then, we use a stack of multi-head self-attention layers to model the spatial and temporal correlations in the sequences. 

%To provide additional supervision signals for mining global correlations, we instruct our model to reconstruct the target frame pixels based on source sequences and select the correct target sequence among a batch of candidates. 
%The goal is to exploit the spatial and temporal correlations in gait recognition and have these supervision signals provide feedback so that the model can learn more discriminative gait features.


%%%%%%% ----------- Figure ------------  %%%%%%%%%%
\begin{figure}[t]
  \centering
  \includegraphics[width=1\linewidth]{fig/Feng/bm_flowchart.pdf}
  \vspace{-6mm}
   \caption{\small Overview of the proposed body shape feature encoding framework. In the body matching process, the identity shape features $\mathbf{z}_{id}$ are utilized for matching.}
   \label{fig:bm_flowchart}
   \vspace{-2mm}
\end{figure}
%%%%%%% ----------- Figure ------------  %%%%%%%%%%

\SubSubSection{Body Shape}
% {\color{red} [Feng, MSU]}
%%
Our method for encoding body features harnesses the power of Person Re-ID~\cite{ye2021deep,ahmed2015improved,zheng2015scalable,li2018harmonious}, with the primary aim to effectively capture static body features. Re-ID can be complex due to variations in human poses and clothing. We propose the naked 3D body shape as the most reliable cue for body matching, despite the considerable challenges in reconstructing it from a 2D image.
%
Taking cues from advancements in 3D feature learning, we introduce a pipeline to disentangle identity (naked body) from non-identity components (pose, clothing shape and texture) of 3D clothed humans. The core of our approach lies in a novel two-layer neural implicit function that disentangles these components in latent representations.

%%
In particular, as illustrated in Fig.~\ref{fig:bm_flowchart}, the proposed method relies on a new joint two-layer neural implicit function that represents $3$D humans, where identity, clothing shape, and texture components are represented in disentangled latent representations.
%
Formally, given a training set of $T$ images $\{\mathbf{I}_i\}_{i=1}^{T}$ and the corresponding identity labels $\{l_i\}_{i=1}^{T}$,
the image encoder $\mathcal{E}(\mathbf{I}):\mathbf{I}\xrightarrow{} (\mathbf{z}_{id}, \mathbf{z}_{cloth}, \mathbf{z}_{tex}$) predicts the identity shape code of naked body $\mathbf{z}_{id}\in\mathbb{R}^{L_{id}}$, clothed shape code $\mathbf{z}_{cloth}\in\mathbb{R}^{L_{cloth}}$ and texture code $\mathbf{z}_{tex}\in\mathbb{R}^{L_{tex}}$. A joint two-layer implicit model decodes the latent codes to identity shape, clothing shape, and texture components, respectively. 
%
Additionally, PoseNet $\mathcal{P}$ predicts the camera projection $\mathbf{\Omega}$ and SMPL body pose $\mathbf{\theta}$: $(\mathbf{\Omega}, \mathbf{\theta}) = \mathcal{P}(\mathbf{I})$.
Mathematically, the learning objective is defined as:
\begin{equation}
\label{eqn:objective}
\argmin_{\mathcal{E},\mathcal{F},\mathcal{C},\mathcal{T}} \sum_{i=1}^T \left(\left|\hat{\mathbf{I}}_i -  \mathbf{I}_i\right|_1 
+ \mathcal{L}_{cla}(\mathbf{z}_{id},l_i)\right),
\end{equation}
where $\mathcal{L}_{cla}$ is the classification loss. $\hat{\mathbf{I}}$ is the rendered image.
%
This objective enables us to jointly learn accurate $3$D clothed shape and discriminative shape for the naked body.

We utilize CAPE~\cite{ma2020learning} and THuman2.0~\cite{zheng2019deephuman} datasets to train our model, generating individual identity shape code, clothing shape code, and texture code for each training sample. For inference, the encoder processes body images to extract identity shape features $\mathbf{z}_{id}$. The Cosine similarity of two $\mathbf{z}_{id}$ determines if two images belong to the same person. This method, excluding the explicit 3D reconstruction during inference, is highly efficient.


%\subsubsection{Multi-Modality Fusion}
\SubSubSection{Multi-Modal Biometric Fusion}
% {\color{red} [Ryan]}
%%
To produce a comprehensive probe-gallery score from multiple biometric modalities, we initially calculate per-modality scores for each probe-gallery pair. For the face, gait, and body, we create a singular subject-level feature using CAFace (Sec.~\ref{face-feature-encoding}), mean fusion on video-only gallery features, and mean fusion on whole-body media, excluding face-only images, respectively. This exclusion is necessary due to the prevalence of face-only gallery images and the unsuitability of gait recognition on single images. 
%For the body, we exclude face-only images by setting a threshold for acceptable vertical padding in preprocessed images.

%%
Probe features are then compared to gallery features, and an equal-weighted sum score fusion is employed to generate a single score from the cosine similarity scores of the three modalities. When feature extraction fails for one or more modalities, we impute missing scores to the middle of the score range, which is zero for the cosine similarity metric used in generating probe-gallery scores.
%
This imputation method was chosen after evaluating alternative techniques, with this approach showing the least bias and greatest stability in our experiments.

%To generate a probe-gallery score from multiple biometric modalities, first per modality scores are computed for all probe-gallery pairs. Each Gallery is represented by a single subject level feature computed for face, gait, and body using CAFace described in Sec. \ref{face-feature-encoding}, mean fusion on video-only gallery features, and mean fusion on whole body media excluding face-only imagery for each modality respectively. Many gallery images focus on the face only, and also the gait feature extraction method is not particularly well suited to single images, which motivates the exclusion of imagery for gait gallery features. For the body, the exclusion of the face-only images is done by thresholding the acceptable amount of vertical padding present in the preprocessed images, as face-only imagery will have body bounding box detections whose bounds extend far beyond the border of the image. Probe features are then compared to these gallery features, and equal-weighted score fusion is applied to generate a single score from the cosine similarity scores of the three modalities.

%Due to the challenging conditions present in long-range, turbulent, and high-angle elevation imagery, it may sometimes be the case that feature extraction may not be successful for one or more modalities for a particular input media. To mitigate the negative impact of missing features and subsequently missing probe-gallery scores, we impute missing scores to the middle of the score metrics range, which is zero for the case of cosine similarity which is the similarity metric used to generate probe-gallery scores.
